Threshold KNN-Shapley: A Linear-Time and Privacy-Friendly Approach to Data Valuation

Data valuation aims to quantify the usefulness of individual data sources in training machine learning (ML) models, and is a critical aspect of data-centric ML research. However, data valuation faces significant yet frequently overlooked privacy challenges despite its importance. This paper studies these challenges with a focus on KNN-Shapley, one of the most practical data valuation methods nowadays. We first emphasize the inherent privacy risks of KNN-Shapley, and demonstrate the significant technical difficulties in adapting KNN-Shapley to accommodate differential privacy (DP). To overcome these challenges, we introduce TKNN-Shapley, a refined variant of KNN-Shapley that is privacy-friendly, allowing for straightforward modifications to incorporate DP guarantee (DP-TKNN-Shapley). We show that DP-TKNN-Shapley has several advantages and offers a superior privacy-utility tradeoff compared to naively privatized KNN-Shapley in discerning data quality. Moreover, even non-private TKNN-Shapley achieves comparable performance as KNN-Shapley. Overall, our findings suggest that TKNN-Shapley is a promising alternative to KNN-Shapley, particularly for real-world applications involving sensitive data.

==> DP_TKNN_shapley.tex <==

\vspace{-3mm}
\section{Differentially Private TKNN-Shapley}
\label{sec:dptknnshapley}

% \tianhao{The privacy analysis could be improved if we do not concern about the membership privacy; the non-collusion assumption will be removed; it becomes joint DP; $\cn$ won't be private statistics anymore so the sensitivity will be reduced to $\sqrt{2}$}

% Having established the TKNN-Shapley method as an alternative to the KNN-Shapley method that shares many advantages, we now turn our attention to further enhancing its privacy guarantees. In the following section, we introduce a differentially private version of TKNN-Shapley (DP-TKNN-Shapley). 

\vspace{-2mm}
Having established TKNN-Shapley as an alternative to KNN-Shapley which shares many advantages, our next step is to develop a new version of TKNN-Shapley that incorporates differential privacy. In this section, we introduce our proposed Differentially Private TKNN-Shapley (DP-TKNN-Shapley). 

\vspace{-2mm}
\subsection{Differentially private release of $\phi^\tknn_{z_i}(\U^\tknn_{ \zval })$} 
\label{sec:dp-tknn-shapley-single}

\vspace{-2mm}
As $\Ct = ( \cn, \ctau, \cA )$ are the only quantities that depend on the dataset $D_{-z_i}$ in (\ref{eq:tknn-shapley}), privatizing these quantities is sufficient for overall privacy preservation, as DP guarantee is preserved under any post-processing \citep{dwork2014algorithmic}. Since all of $\cn, \ctau$ and $\cA$ are just counting queries, the function of $\Ct(\cdot)$  has global sensitivity $\sqrt{3}$ in $\ell_2$-norm. 
This allows us to apply the commonly used Gaussian mechanism (Theorem \ref{thm:gaussian}) to release $\Ct$ in a differentially private way, i.e., 
$\DPCt(D_{-z_i}) := \round \left( \Ct(D_{-z_i}) + \N\left(0, \sigma^2 \ind_3 \right) \right)$
% \vspace{-1mm}
% \begin{small}
% \begin{align*}
% \DPCt(D_{-z_i}) := \round \left( \Ct(D_{-z_i}) + \N\left(0, \sigma^2 \ind_3 \right) \right)
% \end{align*}
% \end{small}
% \vspace{-1mm}
where $\DPCt$ is the privatized version of $\Ct$, and the function $\round$ rounds each entry of noisy value to the nearest integer. 
The differentially private version of TKNN-Shapley value $\widehat \phi^\tknn_{z_i}(D_{-z_i})$ is simply the value score computed by (\ref{eq:tknn-shapley}) but use the privatized quantities $\DPCt$. The privacy guarantee of releasing DP-TKNN-Shapley $\widehat \phi^\tknn_{z_i}(D_{-z_i})$ follows from the guarantee of Gaussian mechanism (see Appendix \ref{appendix:privacy-proof} for proof). 
%\tianhao{refer to appendix; say simplificity as advangtage} 

% If the noisy value is out of range (e.g., $<0$), then it is rounded to the nearest possible value within the valid range. 
% The differentially private version of TKNN-Shapley value $\widehat \phi^\tknn_{z_i}(D_{-z_i}) := \phi^\tknn_{z_i}\left[ \DPCt(D_{-z_i}) \right]$ is simply the value score computed by (\ref{eq:tknn-shapley}) but use the privatized quantities $\DPCt$. 



% % releasing the 3-dimensional vector $\left[ \cn, \ctau, \cA \right]$ has global sensitivity $\sqrt{3}$ in $\ell_2$-norm. This allows us to apply Gaussian mechanism \citep{dwork2006calibrating} for differential privacy, which is one of the most widely used approaches: 
% % \begin{align*}
% % \left[ \DPcn, \DPctau, \DPcA \right] 
% % := \round \left(
% % \left[ \cn, \ctau, \cA \right] + \N\left(0, \sigma^2 \ind_3 \right) \right)
% % \end{align*}
% The function $\round$ rounds a noisy value to the nearest integer. If the noisy value is out of range (e.g., $<0$), then it is rounded to the nearest possible value within the valid range. The differentially private version of TKNN-Shapley value $\widehat \phi^\tknn_{z_i} := \phi^\tknn_{z_i}\left[ \DPcn, \DPctau, \DPcA \right]$ is simply the value score computed by (\ref{eq:tknn-shapley}) but use the privatized quantities $\left[ \DPcn, \DPctau, \DPcA \right]$. 

% We define the differentially private TKNN-Shapley value $\widehat \phi_{z_i}(D_{-z_i}; \zval)$ as the quantity computed based on $\DPctau$ and $\DPcA$. Since both $\DPctau$ and $\DPcA$ are privatized using the Gaussian mechanism, the privacy guarantee of $\widehat \phi_{z_i}$ is ensured by the post-processing property of differential privacy. 

\vspace{-1mm}
\begin{theorem}
\label{thm:privacy-gaussian}
For any $\zval \in \Dval$, releasing 
$
\widehat \phi^\tknn_{z_i}( \U^\tknn_{ \zval } )
:= \phi^\tknn_{z_i}\left[ \DPCt(D_{-z_i}) \right]
$ to data owner $i$ is $(\eps, \delta)$-DP with $\sigma = \sqrt{3} \cdot \sqrt{\log (1.25 / \delta)} / \eps$.
\end{theorem}

% Our approach may strike the readers as being very simple, but we emphasize that the simplicity is generally appreciated in DP for practical deployment. In our humble opinion all problems in DP should admit simple solutions and we are glad to have found one for data valuation.

\vspace{-2mm}
While our approach may seem simple, we stress that simplicity is appreciated in DP as complex mechanisms pose challenges for correct implementation and auditing \citep{lyu2016understanding, gaboardi2020programming}. 

%We believe all DP problems should have simple solutions; we are glad to find one for data valuation.





% \textbf{Differentially private release of $\phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right)$.} Recall that in TKNN-Shapley, the final data value score is $\phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\tknn_{z_i}(D_{-z_i}; \zval)$. We have introduced the mechanism for differentially private releasing $\phi^\tknn_{z_i}(D_{-z_i}; \zval)$ for each $\zval \in \Dval$. 
% We use the composition theorem \citep{dwork2006our} of differential privacy to analyze the privacy guarantee for releasing $\phi^\tknn_{z_i}(D_{-z_i}; \zval)$.

\vspace{-2mm}
\subsection{Advantages of DP-TKNN-Shapley (Overview)}

\vspace{-1mm}
We give an overview (detailed in Appendix \ref{appendix:dp-tknn-detail}) of several advantages of DP-KNN-Shapley here, including the efficiency, collusion resistance, and simplicity in incorporating subsampling. 
% More detailed explanations and derivations can be found in Appendix \ref{appendix:dp-tknn-detail}. 

% \textbf{Efficient computation of DP-TKNN-Shapley by reusing privatized statistics.} 
\vspace{-1mm}
\textbf{By reusing privatized statistics, $\widehat \phi^\tknn_{z_i}$ can be efficiently computed for all $z_i \in D$.} 
Recall that in practical data valuation scenarios, it is often desirable to compute the data value scores for \emph{all of} $z_i \in D$. As we detailed in Section \ref{sec:tknn-shapley}, for TKNN-Shapley, such a computation only requires $O(N)$ runtime in total if we first compute $\Ct(D)$ and subsequently $\Ct(D_{-z_i})$ for each $z_i \in D$. In a similar vein, we can efficiently compute the DP variant $\widehat \phi^\tknn_{z_i}$ for \emph{all} $z_i \in D$. To do so, we first calculate $\DPCt(D)$ and then, for each $z_i \in D$, we compute $\DPCt(D_{-z_i})$. It is important to note that when releasing $\widehat \phi^\tknn_{z_i}$ to individual $i$, the data point they hold, $z_i$, is not private to the individual themselves. 
Therefore, as long as $\DPCt(D)$ is privatized, $\DPCt(D_{-z_i})$ and hence $\widehat \phi^\tknn_{z_i}$ also satisfy the same privacy guarantee due to DP's post-processing property. 

\vspace{-1mm}
\textbf{By reusing privatized statistics, DP-TKNN-Shapley is collusion resistance.} 
In Section \ref{sec:dp-tknn-shapley-single}, we consider the single Shapley value $\phi^\tknn_{z_i}(D_{-z_i})$ as the function to privatize. 
% In Section \ref{sec:dp-tknn-shapley-single}, we consider the release of a single Shapley value $\phi^\tknn_{z_i}(D_{-z_i})$. 
However, when we consider the release of all Shapley values $(\widehat \phi^\tknn_{z_1}, \ldots, \widehat \phi^\tknn_{z_N})$ as a unified mechanism, one can show that such a mechanism satisfies \emph{joint differential privacy} (JDP) \citep{kearns2014mechanism} if we reuse the privatized statistic $\DPCt(D)$ for the release of all $\widehat \phi^\tknn_{z_i}$. The consequence of satisfying JDP is that our mechanism is resilient against collusion among groups of individuals without any privacy degradation. That is, even if an arbitrary group of individuals in $[N] \setminus i$ colludes (i.e., shares their respective $\widehat \phi^\tknn_{z_j}$ values within the group), the privacy of individual $i$ remains uncompromised. Our method also stands resilient in scenarios where a powerful adversary sends multiple data points and receives multiple value scores.

% Additionally, for the scenario where a power adversary who holds multiple data points and receive multiple value scores, the privacy guarantee for the rest of the data points does not degraded. 

% More detailed explanation and derivations can be found in Appendix \ref{appendix:dp-tknn-detail}. 

% This powerful resistance to collusion demonstrates another big advantage of reusing the privatized statistics $\DPCt(D)$. For a more detailed explanation and derivations, we direct the reader to the relevant section in Appendix \ref{appendix:dp-tknn-detail}. 

\vspace{-1mm}
\textbf{Incorporating Privacy Amplification by Subsampling.} In contrast to KNN-Shapley, \add{the non-recursive nature of} DP-TKNN-Shapley allows for straightforward incorporation of subsampling. Besides privacy guarantee, subsampling also significantly boosts the computational efficiency of DP-TKNN-Shapley. % Details can be found in Appendix \ref{appendix:dp-tknn-detail}. 

% \begin{remark}[\textbf{Reusing privatized statistics enables collusion resistance}]
% In Theorem \ref{thm:privacy-gaussian}, we consider $\widehat \phi^\tknn_{z_i}(D_{-z_i})$ for each of $z_i \in D$ as a differentially private mechanism. However, when we consider the release of all Shapley values $(\widehat \phi^\tknn_{z_1}, \ldots, \widehat \phi^\tknn_{z_N})$ as a single, unified mechanism, one can show that such a mechanism satisfies \emph{joint differential privacy} (JDP) \citep{kearns2014mechanism} if we reuse the privatized statistic $\DPCt(D)$ for the release of all $\widehat \phi^\tknn_{z_i}$. The consequence of satisfying JDP is that our mechanism is resilient against collusion among groups of individuals without any privacy degradation. Specifically, if an arbitrary group of individuals that does not include $i$ colludes (i.e., shares their respective $\widehat \phi^\tknn_{z_j}$ values within the group), the privacy of the membership of $z_i$ remains uncompromised. This powerful resistance to collusion demonstrates another big advantage of reusing the privatized statistics $\DPCt(D)$. For a more detailed explanation and derivations, we direct the reader to the relevant section in Appendix \ref{appendix:dp-tknn-detail}. 
% \end{remark}

\vspace{-2mm}
\subsection{Differentially private release of $\phi^\tknn_{z_i}(\U^\tknn_{ \Dval })$} 

%\textbf{Differentially private release of $\phi^\tknn_{z_i}(\U^\tknn_{ \Dval })$ with privacy accounting techniques.}
\vspace{-2mm}
Recall that the TKNN-Shapley corresponding to the full validation set $\Dval$ is $\phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\tknn_{z_i}(D_{-z_i}; \zval)$. 
% We have introduced the mechanism for differentially private releasing $\phi^\tknn_{z_i}(D_{-z_i}; \zval)$ for each $\zval \in \Dval$, and 
We can compute privatized $\phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right)$ by simply releasing $\phi^\tknn_{z_i}(D_{-z_i}; \zval)$ for all $\zval \in \Dval$. To better keep track of the privacy cost, we use the current state-of-the-art privacy accounting technique based on the notion of the Privacy Loss Random Variable (PRV) \citep{dwork2016concentrated}. 
% Here, we provide more details about the background of the compostion of differential privacy and the privacy accounting techniques we use. 
We provide more details about the background of privacy accounting in Appendix \ref{appendix:dp-tknn-detail}. 

% \textbf{Background: Composition of Differential Privacy.} 
% In practice, multiple differentially private mechanisms may be applied to the same dataset, denoted as $\M(D) = \M_1 \circ \M_2 (D) := (\M_1(D), \M_2(D, \M_1(D)))$.\footnote{Multiple DP mechanisms can be \emph{adaptively} composed in the sense that the output of one mechanism can be used as an input to another mechanism.}
% % . Crucially, multiple DP mechanisms can be \emph{adaptively} composed in the sense that the output of one mechanism can be used as an input to another mechanism, denoted as $\M(D) = \M_1 \circ \M_2 (D) := (\M_1(D), \M_2(D, \M_1(D)))$. 
% Differential privacy offers strong composition guarantees, that help quantify the cumulative privacy loss resulting from these combined mechanisms. These guarantees are provided by various composition theorems or privacy accounting techniques, including the basic composition theorem \citep{dwork2006our}, advanced composition theorem \citep{dwork2010boosting}, and Moments Accountant \citep{abadi2016deep}. For example, the basic composition theorem states that if $\M_1$ is $(\eps_1, \delta_1)$-DP and $\M_2$ is $(\eps_2, \delta_2)$-DP, then the composition of $\M_1$ and $\M_2$ is $(\eps_1 + \eps_2, \delta_1 + \delta_2)$-DP. 
% In our scenario, each individual mechanism is the release of $\widehat \phi^\tknn_{z_i}(D_{-z_i}; \zval)$ for each of $\zval \in \Dval$, and we want to keep track of the privacy loss of releasing all of them. 

% \textbf{Privacy Accounting Techniques based on Privacy Loss Random Variable (PRV)}
% To better keep track of the privacy cost, we use the most recent advances in privacy cost accounting based on the notion of the Privacy Loss Random Variable (PRV) \citep{dwork2016concentrated}. The PRV accountant was introduced by \cite{koskela2020computing} and later refined in \cite{koskela2021computing, gopi2021numerical}. 
% For any DP-algorithm, one can easily compute its $(\eps, \delta)$ privacy guarantee based on the distribution of its PRV. The key property of PRVs is that, under (adaptive) composition, they simply add up; the PRV $Y$ of the composition $\M = \M_1 \circ M_2 \circ \dots \circ M_k$ is given by $Y = \sum_{i=1}^k Y_i$, where $Y_i$ is the PRV of $\M_i$. Therefore, one can then find the distribution of $Y$ by convolving the distributions of $Y_1, Y_2, \dots, Y_k$. Prior works \citep{koskela2021computing, gopi2021numerical} approximate the distribution of PRVs by truncating and discretizing them, then using the Fast Fourier Transform (FFT) to efficiently convolve the distributions. 
% In our experiment, we use the FFT-based accountant from \cite{gopi2021numerical}, the current state-of-the-art privacy accounting technique. 



% \textbf{Further boosting privacy-utility tradeoff \& computational efficiency.} 
% Achieving a good privacy-utility tradeoff with differential privacy involves navigating several technical challenges. 
% \textbf{Challenge \#1:} The direct application of the Gaussian mechanism on the full dataset can lead to relatively high privacy costs. 
% \textbf{Challenge \#2:} In order to privately release the Shapley value score evaluated on the full validation set, $\phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\tknn_{z_i}(\zval)$, we must compute $\widehat \phi^\tknn_{z_i}(D_{-z_i}; \zval)$ for each $\zval \in \Dval$. This requires tight privacy loss bounds for the release of $\widehat \phi^\tknn_{z_i}(\zval)$ across all $\zval \in \Dval$. 

% \textbf{Solving Challenge \#1: Privacy Amplification by Subsampling.} 
% In order to further boost the privacy guarantee, we incorporate the privacy amplification by subsampling technique \citep{balle2018privacy}. Specifically, before any computation, we first sample each data point independently with a probability $q$. The differentially private quantities based on the subsampled dataset, denoted as $\subsample(D)$, are calculated as follows:

% \begin{align*}
% \DPcn( D ) &:= \round \left( (1/q) \left( \cn( \subsample(D) ) + \N\left(0, \sigma^2\right) \right) \right) \\
% \DPctau( D ) &:= \round \left( (1/q) \left( \ctau( \subsample(D) ) + \N\left(0, \sigma^2\right) \right) \right) \\
% \DPcA( D ) &:= \round \left( (1/q) \left( \cA( \subsample(D) ) + \N\left(0, \sigma^2\right) \right) \right)
% \end{align*}

% By subsampling the data points, the privacy guarantee is amplified. This is because the subsampling process itself is a randomized operation that provides a level of privacy, making it harder to infer information about individual data points. When combined with the Gaussian mechanism, the overall privacy guarantee is improved. The amplified privacy guarantee can be particularly useful in scenarios where stronger privacy protection is desired or when the dataset contains sensitive information.

% \textbf{Solving Challenge \#2: Tight Privacy Accounting.}
% % \textbf{Releasing Differentially Private TKNN-Shapley $\phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right)$.} 
% Recall that in TKNN-Shapley, the final data value score is $\phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\tknn_{z_i}(D_{-z_i}; \zval)$. We have introduced the mechanism for differentially private releasing $\phi^\tknn_{z_i}(D_{-z_i}; \zval)$ for each $\zval \in \Dval$. 
% We use the composition property of differential privacy to analyze the privacy guarantee for releasing $\phi^\tknn_{z_i}(D_{-z_i}; \zval)$. Specifically, when multiple differentially private mechanisms being applied to the same dataset, the combined mechanism $\M(D) = (\M_1(D), \M_2(D))$ is still differentially private, and the specific privacy guarantee is captured by privacy accounting techniques. 
% In our case, each individual mechanism $\M_i$ corresponds to the release of $\phi^\tknn_{z_i}(\zval)$ for each $\zval \in \Dval$. 
% Various privacy accounting techniques have been proposed \citep{dwork2006our, dwork2010boosting, abadi2016deep}. To better keep track of the privacy cost, we use the current state-of-the-art privacy accounting technique based on the notion of the Privacy Loss Random Variable (PRV) \citep{dwork2016concentrated}. We provide more details about the PRV accountant in Appendix \ref{appendix:background-privacy}. 


% . Crucially, multiple DP mechanisms can be \emph{adaptively} composed in the sense that the output of one mechanism can be used as an input to another mechanism, denoted as $\M(D) = \M_1 \circ \M_2 (D) := (\M_1(D), \M_2(D, \M_1(D)))$. Differential privacy offers strong composition guarantees, that help quantify the cumulative privacy loss resulting from these combined mechanisms. 
% Recall that our final goal is to release $\phi_{z_i}(D_{-z_i}; \Dval) = \sum_{\zval \in \Dval} \phi_{z_i}(D_{-z_i}; \zval)$ in a differentially private way. Hence, in our case, each individual mechanism $\M_i$ corresponds to the release of $\phi_{z_i}(D_{-z_i}; \zval)$ for each $\zval \in \Dval$. 



% \begin{algorithm}[H]
% \SetAlgoLined
% \SetKwInOut{Input}{input}
% \SetKwInOut{Output}{output}

% \Input{Validation dataset $\Dval = \{ \zval = ( x^{(\test)}, y^{(\test)} ) \}$, subsampling rate $q$, noise scale $\sigma$.}

% \For{each $\zval$ in $\Dval$}{
%     Compute $\DPcn(D), \DPctau(D)$ and $\DPcA(D)$ using noise scale $\sigma$ and subsampling rate $q$. \\
%     \For{each $z_i$ in $D$}{
%         Compute $\widehat \phi_{z_i}( D_{-z_i}; \zval)$ using $\DPcn(D), \DPctau( D )$ and $\DPcA( D )$. 
%     }
% }

% \For{each $z_i$ in $D$}{
%     $\widehat \phi_{z_i}( D_{-z_i}; \Dval) \gets \sum_{\zval \in \Dval } \widehat \phi_{z_i}(D_{-z_i}; \zval)$.
% }

% \Return $\widehat \phi_{z_i}( D_{-z_i}; \Dval)$ for all $z_i$.

% \caption{Differentially Private TKNN-Shapley}
% \end{algorithm}



% \subsection{Utility of Gaussian mechanism}

% \begin{theorem}
% Bound 
% \begin{align*}
%     \left|
%     \sum_{ \zval \in \Dval } 
%     \widehat \phi_{z_i}(\zval)
%     - \E\left[ \sum_{ \zval \in \Dval } 
%     \widehat \phi_{z_i}(\zval) \right]
%     \right| 
% \end{align*}
% \end{theorem}


% \subsection{Efficient Implementation}

% As we highlighted earlier, in most of the practical applications, it is desirable to release value scores for \emph{all} data owners in the dataset. To efficiently release DP-TKNN-Shapley scores for all data owners, we adopt two key techniques in the computation process.

% \textbf{Reuse Privatized statistics.} 
% We can reuse the privatized values of $\DPcn, \DPctau$ and $\DPcA$ for all data owners, which reduces the amount of noise introduced and minimizes the privacy budget consumed. By sharing these privatized values among all data owners, we can maintain a consistent level of differential privacy protection while expediting the computation process.





==> TKNN.tex <==

\vspace{-2mm}
\section{The Shapley Value for Threshold-based Nearest Neighbor}

\vspace{-2mm}
Considering the privacy concerns and privatization challenges associated with the original KNN-Shapley method, we introduce \emph{TKNN-Shapley}, a privacy-friendly alternative of KNN-Shapley which also achieves improved computational efficiency. At the core of this novel method is Threshold-KNN (TKNN) classifier, a simple variant of the KNN classifier. 
We will discuss about how to incorporate DP for TKNN-Shapley in Section \ref{sec:dptknnshapley}. 

% Considering the privacy concerns and privatization challenges associated with the original KNN-Shapley method, we introduce \emph{TKNN-Shapley}, a privacy-friendly alternative of KNN-Shapley that retains the same computational efficiency and effectiveness. At the core of this novel method is Threshold-KNN (TKNN) classifier, a simple variant of the KNN classifier. 

% that considers neighbors within a pre-specified threshold of the query example, rather than exclusively focusing on the exact $K$ nearest neighbors. We derive the closed-form, efficiently computable Data Shapley formula for the TKNN classifier (i.e., TKNN-Shapley). TKNN-Shapley not only maintains the computational efficiency and efficacy of KNN-Shapley in evaluating the importance of data points, but also offers the extra advantage of being privacy-friendly. 

% We then redefine the utility function as the soft-label accuracy for TKNN. The refined utility function enables us to develop a more privacy-friendly version of KNN-Shapley, while maintaining the method's efficacy in evaluating the importance of data points in the dataset.

\vspace{-2mm}
\subsection{Threshold-based Nearest Neighbor Classifier (TKNN)}

% \textbf{Motivation.} The sorting nature of searching for exact k-nearest neighbors makes `recursive process` unavoidable. However, our approach eliminates the need for recursion through a simple intuition:``the selection of private data depends solely on the data itself and the validation example, independent of any other private data. To realize this intution, we propose a threshold-base ...

\vspace{-1mm}
Threshold-KNN (TKNN) \citep{bentley1975survey} is a variant of KNN classifier that considers neighbors within a pre-specified threshold of the query example, rather than exclusively focusing on the exact $K$ nearest neighbors. 
Formally, for a training set $S$ and a validation data point $\zval = (x^{(\test)}, y^{(\test)})$, we denote 
$
\NBtauxval(S) 
:= \{(x, y) | (x, y) \in S, d(x, x^{(\test)}) \le \tau \}
$
the set of neighbors of $x^{(\test)}$ in $S$ within a pre-specified threshold $\tau$. 
% , i.e., 
% $
% \NBtauxval(S) 
% := \{(x, y) | (x, y) \in S, d(x, x^{(\test)}) \le \tau \}
% $. 
Similar to the utility function for KNN, we define the utility function for TKNN classifier when using a validation set $\Dval$ as the aggregated prediction accuracy $\U^\tknn_{\Dval}(S) := \sum_{\zval \in \Dval} \U^\tknn_{\zval}(S)$ where 
\begin{small}
\begin{align}
\U^\tknn_{\zval}(S) := 
\begin{cases} 
      \texttt{Constant} & |\NBtauxval(S)|=0 \\
      \frac{1}{ |\NBtauxval(S)| } \sum_{(x, y) \in \NBtauxval(S)} \ind[y = y^{(\test)}] & |\NBtauxval(S)| > 0
\end{cases}
\label{eq:threshold-util}
\end{align}
\end{small}
where $\texttt{Constant}$ can be the trivial accuracy of random guess. 

\textbf{Comparison with standard KNN.} 
\textbf{(1) Robustness to outliers.} Compared with KNN, TKNN is better equipped to deal with prediction phase outliers \citep{bentley1975survey}. When predicting an outlier that is far from the entire training set, TKNN prevents the influence of distant, potentially irrelevant neighbors, leading to a more reliable prediction score for outliers.
%, as it considers only the neighbors within a pre-specified range. 
\textbf{(2) Inference Efficiency.} TKNN has slightly better computational efficiency compared to KNN, as it has $O(N)$ instead of $O(N \log N)$ inference time. This improvement is achieved because TKNN only requires the computation of neighbors within the threshold $\tau$, rather than searching for the exact $K$ nearest neighbors. 
\textbf{(3) TKNN is also a consistent estimator.} The consistency of standard KNN is a well-known theoretical result \citep{gyorfi2002distribution}. That is, for any target function that satisfies certain regularity conditions, KNN binary classifier/regressor is guaranteed to converge to the target function as the size of the training set grows to infinite. In Appendix \ref{appendix:consistency}, we derived a similar consistency result for TKNN binary classifier/regressor. 

% \textbf{Why we consider TKNN?} 


\vspace{-1mm}
\subsection{Data Shapley for TKNN (TKNN-Shapley)}
\label{sec:tknn-shapley}

\vspace{-1mm}
With the introduction of TKNN classifier and its utility function, we now present our main result, the closed-form, efficiently computable Data Shapley formula for the TKNN classifier.

% By leveraging the utility function presented in Equation (\ref{eq:threshold-util}), we can express the Shapley value of each training point $z_i = (x_i, y_i) \in D$ for TKNN as follows:

\begin{theorem}[TKNN-Shapley (simplified version)]
\label{thm:TKNN-shapley}
Consider the utility function $\U^\tknn_{\zval}$ in (\ref{eq:threshold-util}). 
Given a validation data point $\zval = (x^{(\test)}, y^{(\test)})$ and a distance metric $d(\cdot, \cdot)$, the Shapley value $\phi^\tknn_{z_i}$ of each training point $z_i = (x_i, y_i) \in D$ corresponding to utility function $\U^\tknn_{\zval}$ can be calculated as 
\begin{small}
\begin{align}
\phi^\tknn_{z_i} = f\left( \Ct(D_{-z_i}) \right)
\label{eq:tknn-shapley}
\end{align}
\end{small}
where $\Ct := ( \cn, \ctau, \cA )$ is a 3-dimensional function/vector s.t. 
\begin{small}
\begin{align*}
    \cn &= \cn(D_{-z_i}) := |D_{-z_i}|  & (\text{size of}~D_{-z_i}) \\
    \ctau &= \ctau( D_{-z_i} ) := 1 +  \left| \NBtauxval( D_{-z_i} ) \right|  & (1+\text{\# neighbors of}~\xval~\text{in}~D_{-z_i}) \\ 
    \cA &= \cA( D_{-z_i} ) := \sum_{(x, y) \in \NBtauxval( D_{-z_i} )} \ind[y = y^{(\test)}] & (\text{\# same-label neighbors in}~D_{-z_i})
\end{align*}
\end{small} 
and $f(\cdot)$ is a function whose exact form can be found in Appendix \ref{appendix:tknn-detail}. 

\vspace{-0.5mm}
\emph{\textbf{Runtime:}} the computation of all $(\phi^\tknn_{z_1}, \ldots, \phi^\tknn_{z_N})$ can be achieved in $O(N)$ runtime \add{(see Appendix \ref{appendix:tknn-shapley-fullversion})}. 

\vspace{-0.5mm}
\emph{\textbf{The Shapley value when using full validation set:}} The Shapley value corresponding to the utility function $\U^\tknn_{\Dval}$ 
% on the overall validation set $\Dval$ 
can be calculated as 
$
\phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\tknn_{z_i} \left( \U^\tknn_{\zval} \right)
$. 
\end{theorem}


% follows: 
% \begin{small}
% \begin{align}
%     \phi^\tknn_{z_i} = 
%     \begin{cases} 
%     \ind[\ctau \ge 2] A_1 A_2 
%     + \frac{ \ind[y_i = y^{(\test)}] - 1/C }{\ctau}
%     & d(x_i, x^{(\test)}) \le \tau \\
%     0 & d(x_i, x^{(\test)}) > \tau
%     \end{cases}
%     \label{eq:tknn-shapley}
% \end{align}
% \end{small}
% where 
% $
% A_1 = \frac{\ind[y_i = y^{(\test)}]}{\ctau} - \frac{\cA}{\ctau (\ctau-1)}
% $, 
% $
% A_2 =
%     \sum_{k=0}^{ \cn } \left[ \frac{1}{k+1} - \frac{1}{k+1} \cdot \frac{ { \cn - k \choose \ctau} }{ { \cn+1  \choose \ctau} } \right] - 1 
% $, 
% % \begin{small}
% % \begin{align*}
% %     A_1 &= \frac{\ind[y_i = y^{(\test)}]}{\ctau} - \frac{\cA}{\ctau (\ctau-1)}, ~~~ A_2 =
% %     \sum_{k=0}^{ \cn } \left[ \frac{1}{k+1} - \frac{1}{k+1} \cdot \frac{ { \cn - k \choose \ctau} }{ { \cn+1  \choose \ctau} } \right] - 1 
% % \end{align*}
% % \end{small}

% and
% \begin{small}
% \begin{align*}
%     \cn &= \cn(D_{-z_i}) := |D_{-z_i}| \\
%     \ctau &= \ctau( D_{-z_i} ) := \left| \NBtauxval( D_{-z_i} ) \right| + 1,\\ 
%     \cA &= \cA( D_{-z_i} ) := \sum_{(x, y) \in \NBtauxval( D_{-z_i} )} \ind[y = y^{(\test)}]
% \end{align*}
% \end{small}
% The Shapley value corresponding to the utility function $\U^\tknn_{\Dval}$ on the overall validation set $\Dval$ can be calculated as 
% $
% \phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\tknn_{z_i} \left( \U^\tknn_{\zval} \right)
% $. 
% \end{theorem}

% \begin{theorem}[TKNN-Shapley]
% \label{thm:TKNN-shapley}
% Consider the utility function in (\ref{eq:threshold-util}). Given the test data point $(x^{(\test)}, y^{(\test)})$, the Shapley value $\phi_{z_i}$ of each training point $z_i = (x_i, y_i) \in D$ can be calculated as follows: 
% \begin{small}
% \begin{align*}
%     &\phi_{z_i}(D_{-z_i}; (x^{(\test)}, y^{(\test)})) \\
%     &= 
%     \begin{cases} 
%     \ind[\ctau \ge 2] 
%     \left( \frac{\ind[y_i = y^{(\test)}]}{\ctau} - \frac{\cA}{\ctau (\ctau-1)} \right) \left(
%     \sum_{k=0}^{N-1} \left[ \frac{1}{k+1} - \frac{1}{k+1} \cdot \frac{ {N-1-k \choose \ctau} }{ {N \choose \ctau} } \right] - 1
%     \right) 
%     + \frac{ \ind[y_i = y^{(\test)}] - 1/C }{\ctau}
%     & d(x_i, x^{(\test)}) \le \tau \\
%     0 & d(x_i, x^{(\test)}) > \tau
%     \end{cases}
% \end{align*}
% \end{small}
% where 
% \begin{align*}
%     \ctau &= \ctau( D_{-z_i} ) := \left| \NBtauxval( D_{-z_i} ) \right| + 1,\\ 
%     % \cA &= \cA( D_{-z_i} ) := \sum_{(x, y) \in \NBtauxval(D)} \ind[y = y^{(\test)}] - \ind[y_i = y^{(\test)}]
%     \cA &= \cA( D_{-z_i} ) := \sum_{(x, y) \in \NBtauxval( D_{-z_i} )} \ind[y = y^{(\test)}]
% \end{align*}
% \end{theorem}


% \textbf{Comparison against KNN-Shapley: 
% Computational Efficiency and Non-recursive Nature.} 
% The TKNN-Shapley method offers an advantage in terms of computational efficiency compared to KNN-Shapley. The summation term $\sum_{j=0}^{N-1} \left[ \frac{1}{j+1} - \frac{1}{j+1} \cdot \frac{ {N-1-j \choose \ctau} }{ {N \choose \ctau} } \right]$ can be computed in $O(N)$ time. Since this term is independent of $i$, it can be reused across all data points $i$, leading to an overall computational cost of $O(N)$ for calculating the Shapley values of all data points $(\phi_{z_i})_{i=1}^N$. In contrast, the KNN-Shapley method has a computational cost of $O(N\log N)$, as it requires sorting the training data according to their distance to the validation data. 
% Furthermore, unlike the KNN-Shapley method, which is based on a recursive formula, the TKNN-Shapley method provides an explicit formula for the Shapley value of every data point $z_i$. This non-recursive nature simplifies the computation process. 

% Similar to KNN-Shapley, after computing the Data Shapley score $\phi^\tknn_{z_i} \left(\U^\tknn_{\zval} \right)$ for each $\zval \in \Dval$, the Data Shapley corresponding to the utility function $\U_{\Dval}$ on the overall validation set $\Dval$ can be determined using the linearity axiom of the Shapley value, i.e., 
% $
% \phi^\tknn_{z_i} \left(\U^\tknn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\tknn_{z_i} \left( \U^\tknn_{\zval} \right)
% $. 

% Moreover, from Theorem \ref{thm:TKNN-shapley} we can see that $\cn, \ctau$ and $\cA$ are the key quantities for computing $\phi^\tknn_{z_i}$, we sometimes view $\phi^\tknn_{z_i}$ as a function of these three quantities and write $\phi^\tknn_{z_i}\left[ \cn, \ctau, \cA \right]$ when we want to stress this dependency. 

\vspace{-1mm}
The main technical challenges of proving Theorem \ref{thm:TKNN-shapley} lies in showing $\Ct = ( \cn, \ctau, \cA )$, three simple counting queries on $D_{-z_i}$, are the key quantities for computing $\phi^\tknn_{z_i}$. 
In later part of the paper, we will often view $\phi^\tknn_{z_i}$ as a function of $\Ct$ and denote $\phi^\tknn_{z_i}\left[ \Ct \right] := f( \Ct )$ when we want to stress this dependency. 
% Moreover, we denote $\Ct(D) := \left( \cn(D), \ctau(D), \cA(D) \right)$ when we want to stress that these statistics are computed for the dataset $D$. 
The full version and the proof for TKNN-Shapley can be found in Appendix \ref{appendix:tknn-detail}. Here, we briefly discuss why TKNN-Shapley can achieve $O(N)$ runtime \emph{in total}. 

\vspace{-1mm}
\textbf{Efficient Computation of TKNN-Shapley.} As we can see, all of the quantities in $\Ct$ are simply counting queries on $D_{-z_i}$, and hence $\Ct(D_{-z_i})$ can be computed in $O(N)$ runtime for any $z_i \in D$. A more efficient way to compute $\Ct(D_{-z_i})$ for \emph{all} $z_i \in D$, however, is to first compute $\Ct(D)$ on the full dataset $D$, and we can easily show that each of $\Ct(D_{-z_i})$ can be computed from that in $O(1)$ runtime (see Appendix \ref{appendix:tknn-detail} for details). 
Hence, we can compute TKNN-Shapley $\phi^\tknn_{z_i}(\U^\tknn_{\zval})$ for \emph{all} $z_i \in D$ within an overall computational cost of $O(N)$. 

\vspace{-1mm}
\textbf{Comparison with KNN-Shapley.} TKNN-Shapley offers several advantages over the original KNN-Shapley. 
\textbf{(1) Non-recursive:} In contrast to the KNN-Shapley formula (Theorem \ref{thm:knn-shapley}), which is recursive, TKNN-Shapley has an explicit formula for computing the Shapley value of every point $z_i$. This non-recursive nature not only simplifies the implementation, but also makes it straightforward to incorporate techniques like subsampling. 
\textbf{(2) Computational efficiency:} TKNN-Shapley has $O(N)$ runtime in total, which is better than the $O(N \log N)$ runtime for KNN-Shapley. 

% Hence, we can compute TKNN-Shapley $\phi^\tknn_{z_i}(\U^\tknn_{\zval})$ for \emph{all of} $z_i \in D$ within an overall computational cost of $O(N)$. 
% In contrast, the KNN-Shapley has a computational cost of $O(N\log N)$, as it requires sorting the training data according to their distances to the validation data. 

% % since 
% % \begin{align*}
% % \Ct(D_{-z_i}) = \Ct(D) + ( 0, \ind[ d(x_i, x^{(\test)}) \le \tau ] , \ind[ d(x_i, x^{(\test)}) \le \tau \text{~and~} \ind[y_i = y^{(\test)}] ] )
% % \end{align*}
% Hence, we can compute TKNN-Shapley $\phi^\tknn_{z_i}(\U^\tknn_{\zval})$ for \emph{all of} $z_i \in D$ within an overall computational cost of $O(N)$. 
% % both the quantities of $\ctau(D_{-i}), \cA(D_{-i})$ can be computed in $O(N)$ runtime. 
% % More importantly, we can first compute $(\cn(D), \ctau(D), \cA(D))$ for the full dataset $D$, and each of $(\cn(D_{-i}), \ctau(D_{-i}), \cA(D_{-i}))$ can be computed from that in $O(1)$ extra runtime. 
% % % Moreover, we can compute $(\ctau(D_{-j}), \cA(D_{-j}))$ from $(\ctau(D_{-i}), \cA(D_{-i}))$ for any $j \ne i$ with $O(1)$ extra runtime. 
% % Hence, we can compute TKNN-Shapley $\phi^\tknn_{z_i}(\U^\tknn_{\zval})$ for \emph{all of} $z_i \in D$ within an overall computational cost of $O(N)$. 
% % % $\phi^\tknn_{z_i}((x^{(\test)}, y^{(\test)}))$ can be computed in $O(N)$ time. Since this term is independent of $i$, it can be reused across all data points $i$, leading to an overall computational cost of $O(N)$ for calculating the Shapley values of all data points $(\phi_{z_i})_{i=1}^N$. 
% In contrast, the KNN-Shapley has a computational cost of $O(N\log N)$, as it requires sorting the training data according to their distances to the validation data. 

%\textbf{(2) Non-recursive:} Unlike the KNN-Shapley in Theorem \ref{thm:knn-shapley}, which is a recursive formula, the TKNN-Shapley method provides an explicit formula for the Shapley value of every data point $z_i$. This non-recursive nature simplifies the implementation. 
% \textbf{(3) Efficient Online Data Valuation:} TKNN-Shapley enables efficient online data valuation. When a new training data point arrives, it allows for the efficient update $\cn, \ctau$ and $\cA$, which means that the data value scores for the existing training data points can be updated in $O(1)$ time, and the value of the new training data point can be computed in $O(1)$ time. 
% %of the existing training data points, as well as the efficient computation of the value of the new training data point. 
% This capability is beneficial in scenarios where the dataset is constantly evolving or expanding, as it avoids the need for recalculating the Shapley values for all data points from scratch.



==> conclusion.tex <==

\vspace{-3mm}
\section{Conclusion}

\vspace{-2mm}
In this work, we uncover the inherent privacy risks associated with data value scores and introduce TKNN-Shapley, a privacy-friendly alternative to the widely-used KNN-Shapley. 
We demonstrate that TKNN-Shapley outperforms KNN-Shapley in terms of computational efficiency, and is as good as discerning data quality. 
Moreover, the privatized version of TKNN-Shapley significantly surpasses the naively privatized KNN-Shapley on tasks such as mislabeled data detection. 

\vspace{-1mm}
\textbf{Limitations \& Future Work.} 
\textbf{(1) Privacy risks of data revelation to central server:} in this work, we assume the existence of a trusted central server, and we do not consider the privacy risks associated with revealing individuals' data to the central server. Future work should consider integrating secure multi-party computation (MPC) techniques to mitigate this risk \citep{tian2022private}. 
% MPC can allow the computation of KNN-Shapley without revealing individual data to the central server, thereby preserving privacy. 
We envision an end-to-end privacy-preserving data valuation framework that combines both DP and MPC. \textbf{(2) Impact of Randomization on Payment Fairness:} the incorporation of differential privacy necessarily adds a degree of randomness to the data value scores. This randomization could potentially impact the fairness of payments to data providers \citep{bagdasaryan2019differential}. The influence of this randomness, and its potential implications for payment fairness, remain areas for further investigation. 
% \tianhao{ add citation for Shapley axiom; dp for fairness }
% Future research could explore strategies for balancing the need for privacy protection with the goal of fair compensation for data providers.




% This work considers the central DP setting and privatizes $\phi^\tknn_{z_i}(D_{-z_i})$ to protect the privacy of \emph{membership} within $D_{-z_i}$. As we highlighted earlier, such a strong privacy notion requires individuals not to share their privatized data value scores with others. However, in some practical data valuation scenarios, membership might not constitute sensitive information, but the data held by individuals does. Under such circumstances, it could be beneficial to develop a new, relaxed privacy notion, akin to label differential privacy \citep{ghazi2021deep}. This revised privacy framework could potentially permit the sharing of privatized data value scores while still safeguarding the privacy of the data information held by individuals.
% \tianhao{randomness}

% In this work, we uncover the inherent privacy risks in data value scores and present TKNN-Shapley, a privacy-friendly and computationally efficient alternative to the famous KNN-Shapley. We demonstrate that TKNN-Shapley matches or even surpasses KNN-Shapley in computational efficiency and discerning data quality in non-private settings, and its privatized version significantly outperforms the naively privatized KNN-Shapley in private settings. 

% \textbf{Limitations \& Future Work.} In this work, we consider the central DP setting, and we privatize $\phi^\tknn_{z_i}(D_{-z_i})$ in order to protect the privacy of members in $D_{-z_i}$. As we mentioned earlier, such a strong notion of privacy requires different individuals not share the privatized data value scores with each other. In some practical scenario of data valuation, membership may not be a sensitive information, but the data hold by the individuals are. In this case, we can potentially develop a new, relaxed privacy notion similar to label differential privacy \citep{ghazi2021deep} which can potentially allow the sharing of privatized data value scores while protecting the privacy of the data information hold by individuals. 


==> experiment.tex <==

\vspace{-2mm}
\section{Numerical Experiments}
\label{sec:eval}


\vspace{-2mm}
In this section, we systematically evaluate the practical effectiveness of our proposed TKNN-Shapley method. Our evaluation aims to demonstrate the following points: 
\textbf{(1)} TKNN-Shapley offers \ul{improved runtime efficiency} compared with KNN-Shapley. 
\textbf{(2)} The differentially private version of TKNN-Shapley (DP-TKNN-Shapley) achieves \ul{significantly better privacy-utility tradeoff} compared to naively privatized KNN-Shapley. 
\textbf{(3)} Non-private TKNN-Shapley maintains a \ul{comparable performance} to the original KNN-Shapley in discerning data quality. 
These observations highlight TKNN-Shapley's potential for data valuation in real-life applications. 
Detailed settings for our experiments are provided in Appendix \ref{appendix:experiment}. 


% \textbf{(3)} The differentially private version of TKNN-Shapley (DP-TKNN-Shapley) achieves \ul{significantly better privacy-utility tradeoff} compared to naively privatized KNN-Shapley, highlighting its potential for data valuation in real-life applications. 
% Detailed settings for our experiments are provided in Appendix \ref{appendix:experiment}. 




% In this section, we systematically investigate the practical effectiveness of the proposed TKNN-Shapley method through three sets of experiments, which are
% frequently used in previous studies: mislabeled data detection, noisy data detection, and point removal experiment. 
% Our evaluation aims to illustrate the following points: 
% \textbf{(1) In non-private setting: } TKNN-Shapley maintains a similar performance and computational efficiency as the original KNN-Shapley (and outperforms the traditional retrain-based data valuation techniques); 
% \textbf{(2) In private setting:} TKNN-Shapley achieves significantly better performance than KNN-Shapley. 
% Detailed settings are provided in Appendix \ref{appendix:experiment}. 

\vspace{-2mm}
\subsection{Computational Efficiency}
\label{sec:eval-runtime}

\vspace{-1mm}

\begin{wrapfigure}{R}{0.35 \textwidth}
    \setlength\intextsep{0pt}
    \setlength\abovecaptionskip{0pt}
    \setlength\belowcaptionskip{-20pt}
    \vspace{-4mm}
    \centering
    \includegraphics[width=0.35 \columnwidth]{image/runtime.pdf}
    \caption{ Runtime comparison of TKNN-Shapley and KNN-Shapley across various training data sizes $N$. The plot shows the average runtime based on 5 independent runs. Experiments were conducted with an AMD 64-Core CPU Processor.
    }
    \label{fig:runtime}
\end{wrapfigure}
We evaluate the runtime efficiency of TKNN-Shapley in comparison to KNN-Shapley using a synthetic dataset generated from a Gaussian distribution (see Appendix \ref{appendix:experiment} for details as well as more experiments). We choose a range of training data sizes $N$, and compare the runtime of both methods at each $N$. As demonstrated in Figure \ref{fig:runtime}, TKNN-Shapley achieves better computational efficiency than KNN-Shapley across all training data sizes. In particular, TKNN-Shapley is around 30\% faster than KNN-Shapley for large $N$. 
This shows the computational advantage of TKNN-Shapley mentioned in Section \ref{sec:tknn-shapley}. 

% The improvement in runtime efficiency is because TKNN-Shapley does not require sorting $N$ data points, which saves a factor of $O(\log N)$ in runtime complexity compared with KNN-Shapley. 

% can be attributed to the fact that TKNN-Shapley has an $O(N)$ runtime complexity, while KNN-Shapley's runtime complexity is $O(N \log N)$.


% \begin{table}[t]
% \setlength\intextsep{0pt}
% \setlength\abovecaptionskip{0pt}
% \setlength\belowcaptionskip{-10pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}ccccccc@{}} \toprule
%                     & \multicolumn{3}{c}{\textbf{Mislabeled Detection}}                    & \multicolumn{3}{c}{\textbf{Noisy Data Detection}}                    \\ \midrule
% \textbf{Dataset}    & \textbf{TKNN-Shapley} & \textbf{KNN-Shapley} & \textbf{Data Shapley} & \textbf{TKNN-Shapley} & \textbf{KNN-Shapley} & \textbf{Data Shapley} \\ \midrule
% \textbf{2DPlanes}   & 0.919 (0.006)         & 0.913                & 0.552                 & 0.711 (0.141)         & 0.57                 & 0.545                 \\
% \textbf{Fraud}      & 0.96 (-0.007)         & 0.967                & 0.488                 & 0.854 (0.232)         & 0.622                & 0.502                 \\
% \textbf{Creditcard} & 0.662 (0.016)         & 0.646                & 0.517                 & 0.608 (0.064)         & 0.544                & 0.535                 \\
% \textbf{Vehicle}    & 0.737 (-0.122)        & 0.859                & 0.552                 & 0.626 (0.017)         & 0.609                & 0.544                 \\
% \textbf{Apsfail}    & 0.958 (0.01)          & 0.948                & 0.496                 & 0.867 (0.272)         & 0.595                & 0.533                 \\
% \textbf{Click}      & 0.572 (0.004)         & 0.568                & 0.474                 & 0.545 (0.015)         & 0.53                 & 0.461                 \\
% \textbf{Phoneme}    & 0.826 (-0.047)        & 0.873                & 0.525                 & 0.709 (0.119)         & 0.59                 & 0.49                  \\
% \textbf{Wind}       & 0.889 (-0.007)        & 0.896                & 0.469                 & 0.776 (0.157)         & 0.619                & 0.495                 \\
% \textbf{Pol}        & 0.871 (-0.057)        & 0.928                & 0.512                 & 0.712 (0.1)           & 0.612                & 0.526                 \\
% \textbf{CPU}        & 0.946 (0.014)         & 0.932                & 0.489                 & 0.786 (0.169)         & 0.617                & 0.527                 \\
% \textbf{MNIST}      & 0.962 (-0.012)        & 0.974                & -                     &                       & 0.815                & -                     \\
% \textbf{CIFAR10}    & 0.957 (-0.034)        & 0.991                & -                     &                       &                      & -                     \\
% \textbf{AG News}    & 0.956 (-0.015)        & 0.971                & -                     &                       & 0.746                & -                     \\
% \textbf{DBPedia}    & 0.981 (-0.01)         & 0.991                & -                     &                       & 0.88                 & -                     \\ \bottomrule     
% \end{tabular}
% }
% \caption{AUROC scores of TKNN/KNN-Shapley and Data Shapley for mislabeled/noisy data detection tasks on various datasets. The higher the AUROC score is, the better the method is. In the column for TKNN-Shapley, we highlight its performance difference with KNN-Shapley in the $()$. 
% The results for Data Shapley on the last 4 datasets are omitted due to computational constraints. 
% }
% \label{tb:non-private}
% \end{table}


\vspace{-2mm}
\subsection{Discerning Data Quality}

\vspace{-1mm}
In this section, we evaluate the performance of both DP and non-DP version of TKNN-Shapley in discerning data quality. 
\textbf{\underline{Tasks:}} We evaluate the performance of TKNN-Shapley on two standard tasks: \uline{mislabeled data detection} and \uline{noisy data detection}, which are tasks that are often used for evaluating the performance of data valuation techniques in prior works \citep{kwon2022beta, wang2023data}. Since mislabeled/noisy data often negatively affect the model performance, it is desirable to assign low values to these data points. In the experiment of mislabeled (or noisy) data detection, we randomly choose 10\% of the data points and flip their labels (or add strong noise to their features). 
% For the task of mislabeled data detection, we randomly choose 10\% of the entire data points and change their labels to one of the other labels. For the task of noisy data detection, we randomly choose 10\% of the data points and add strong white noise to their features. 
% These tasks are frequently used in the prior works \citep{kwon2022beta, wang2023data} for evaluating the reliability of data value scores. 
% ability of data valuation methods to identify bad data points that could adversely impact the model's performance. 
\underline{\textbf{Datasets:}} We conduct our experiments on a diverse set of 13 datasets, where 11 of them have been used in previous data valuation studies \citep{kwon2022beta, wang2023data}. Additionally, we experiment on 2 NLP datasets (AG News \citep{wang2021n24news} and DBPedia \citep{auer2007dbpedia}) that have been rarely used in the past due to their high-dimensional nature and the significant computational resources required. 
\underline{\textbf{Settings \& Hyperparameters of TKNN-/KNN-Shapley:}} for both TKNN/KNN-Shapley, we use the popular cosine distance as the distance measure \citep{knntutorial}, which is always bounded in $[-1, +1]$. 
Throughout all experiments, we use $\tau = -0.5$ and $K=5$ for TKNN-/KNN-Shapley, respectively, as we found the two choices consistently work well across all datasets. We conduct ablation studies on the choice of hyperparameters in Appendix \ref{appendix:ablation}. 



% \begin{wrapfigure}{R}{0.6 \textwidth}
%     \setlength\intextsep{0pt}
%     \setlength\abovecaptionskip{0pt}
%     \setlength\belowcaptionskip{-10pt}
%     \vspace{-5mm}
%     \centering
%     \includegraphics[width=0.6 \columnwidth]{image/2dplanes_tradeoff.pdf}
%     \caption{ 
%     Privacy-utility tradeoff of DP-TKNN-Shapley and DP-KNN-Shapley for (a) mislabeled and (b) noisy data detection task. The curves show the AUROC at different privacy budget $\eps$; the higher the curve is, the better the method is. The error bar is the standard deviation of AUROC across 5 independent runs. 
%     }
%     \label{fig:privacy-tradeoff}
% \end{wrapfigure}



\vspace{-2mm}
\subsubsection{Experiment for Private Setting}
\label{sec:eval-privacy}
\vspace{-1mm}
\underline{\textbf{Baselines:}} 
\textbf{(1) DP-KNN-Shapley without subsampling.} 
Recall from Section \ref{sec:difficulty-in-privatize-knn}, the original KNN-Shapley has a large global sensitivity. 
% it is not easy to bound global sensitivity of KNN-Shapley. Hence, we use the older version of KNN-Shapley from \citep{jia2019efficient} where the global sensitivity can be bounded (but still large), and 
Nevertheless, we can still use Gaussian mechanism to privatize it based on its global sensitivity bound. We call this approach as DP-KNN-Shapley and is detailed in Appendix \ref{appendix:background-more}. 
\textbf{(2) DP-KNN-Shapley with subsampling.} Recall from Section \ref{sec:difficulty-in-privatize-knn}, it is computationally expensive to incorporate subsampling techniques for DP-KNN-Shapley (detailed in Appendix \ref{appendix:background-more}). For instance, subsampled DP-KNN-Shapley with subsampling rate $q=0.01$ generally takes {$\mathbf{30\times}$\textbf{longer time} compared with non-subsampled counterpart. Nevertheless, we still compare with subsampled DP-KNN-Shapley for completeness. 
We also note that an unpublished manuscript \citep{watson2022differentially} proposed a DP version of Data Shapley. However, their DP guarantee requires hard-to-verify assumption of uniform stability (see Appendix \ref{appendix:relatedwork}). %, and they only provide limited experiment details. 
Hence, we do not compare with \citep{watson2022differentially}. 


\vspace{-1mm}
\underline{\textbf{Results:}} We evaluate the privacy-utility tradeoff of DP-TKNN-Shapley. 
Specifically, for a fixed $\delta$, we examine the AUROC of mislabeled/noisy data detection tasks at different values of $\eps$, where $\eps$ is adjusted by changing the magnitude of Gaussian noise. 
In the experiment, we set the subsampling rate $q=0.01$ for TKNN-Shapley and subsampled KNN-Shapley. Table \ref{tb:privacy-tradeoff} shows the results on 3 datasets, and we defer the results for the rest of 10 datasets to Appendix \ref{appendix:experiment}. As we can see, \ul{\textbf{DP-TKNN-Shapley shows a substantially better privacy-utility tradeoff compared to both DP-KNN-Shapley with/without subsampling.}} In particular, DP-TKNN-Shapley maintains a high AUROC even when $\eps \approx 0.1$. The poor performance of DP-KNN-Shapley is due to its relatively high global sensitivity. 


\input{table_privacy}


\vspace{-2mm}
\subsubsection{Experiment for Non-private Setting} 

\begin{wraptable}{r}{0.5 \columnwidth}
\vspace{-4mm}
\setlength\intextsep{0pt}
\setlength\abovecaptionskip{2pt}
\setlength\belowcaptionskip{-10pt}
\resizebox{0.5 \textwidth}{!}{
\begin{tabular}{cccc} \toprule
\textbf{Dataset}    & \textbf{TKNN-Shapley} & \textbf{KNN-Shapley} & \textbf{Data Shapley} \\ \midrule
\textbf{2dPlanes}   & 0.919 \red{(+0.006)}         & 0.913                & 0.552                 \\
\textbf{Phoneme}    & 0.826 \red{(-0.047)}        & 0.873                & 0.525                 \\
\textbf{CPU}        & 0.946 \red{(+0.014)}         & 0.932                & 0.489                 \\
\textbf{Fraud}      & 0.96 \red{(-0.007)}         & 0.967                & 0.488                 \\
\textbf{Creditcard} & 0.662 \red{(+0.016)}         & 0.646                & 0.517                 \\
% \textbf{Vehicle}    & 0.737 (-0.122)        & 0.859                & 0.552                 \\
\textbf{Apsfail}    & 0.958 \red{(+0.01)}          & 0.948                & 0.496                 \\
\textbf{Click}      & 0.572 \red{(+0.004)}         & 0.568                & 0.474                 \\
\textbf{Wind}       & 0.889 \red{(-0.007)}        & 0.896                & 0.469                 \\
\textbf{Pol}        & 0.871 \red{(-0.057)}        & 0.928                & 0.512                 \\
\textbf{MNIST}      & 0.962 \red{(-0.012)}        & 0.974                & -                     \\
\textbf{CIFAR10}    & 0.957 \red{(-0.034)}        & 0.991                & -                     \\
\textbf{AG News}    & 0.956 \red{(-0.015)}        & 0.971                & -                     \\
\textbf{DBPedia}    & 0.981 \red{(-0.01)}         & 0.991                & -                     \\ \hline
\end{tabular}
}
\caption{
AUROC scores of TKNN/KNN-Shapley and Data Shapley for mislabeled data detection tasks on various datasets. The higher the AUROC score is, the better the method is. In the column for TKNN-Shapley, we highlight its performance difference with KNN-Shapley in \red{()}. 
The results for Data Shapley on the last 4 datasets are omitted due to computational constraints. 
}
\label{tb:non-private}
\end{wraptable}


\vspace{-1mm}
\underline{\textbf{Baselines:}} Our main baseline for comparison is KNN-Shapley. For completeness, we also compare with other classic, yet much less efficient data valuation techniques, such as Data Shapley \citep{ghorbani2019data}, Data Banzhaf \citep{wang2023data}, and leave-one-out error (LOO) \citep{koh2017understanding}. Due to space constraints, we only show the results for the famous Data Shapley here and defer other methods' results to Appendix \ref{appendix:experiment}. 

\vspace{-1mm}
\underline{\textbf{Results:}} We use AUROC as the performance metric on mislabeled/noisy data detection tasks. 
% for different data valuation techniques. 
Due to space constraints, we defer the results for the task of noisy data detection to Appendix \ref{appendix:experiment}. 
Table \ref{tb:non-private} shows the results for the task of mislabeled data detection across all 13 datasets we use. 
As we can see, \ul{\textbf{TKNN-Shapley shows a comparable performance as KNN-Shapley}} across almost all datasets, demonstrating that TKNN-Shapley matches the effectiveness of KNN-Shapley in discerning data quality. 
Moreover, KNN-Shapley (and TKNN-Shapley) has a significantly better performance compared to Data Shapley, which is consistent with the observations in many existing studies \citep{jia2019scalability, pandl2021trustworthy}. 
The poor performance of Data Shapley is attributable to the sample inefficiency and stochasticity during retraining \citep{wang2023data}. 

% and there are two takeaways: 
% \ul{\textbf{(1) TKNN-Shapley shows a comparable performance as KNN-Shapley for mislabeled data detection.}} This is consistent across almost all datasets, highlighting that TKNN-Shapley is at least as effective as KNN-Shapley in discerning data quality. 
% \ul{\textbf{(2) TKNN-Shapley shows significantly better performance than KNN-Shapley on noisy data detection.}} This superior performance can be attributed to the fact that TKNN is almost guaranteed to assign 0 value to noisy data points that are far from the population, while for KNN-Shapley the values it assigns to noisy data points are less predictable. Moreover, KNN-Shapley (and TKNN-Shapley) has significantly better performance compared to Data Shapley, which is consistent with the observations in many existing studies \citep{jia2019scalability, pandl2021trustworthy}. 






% In the experiment, we set the subsampling rate $q=0.01$ for TKNN-Shapley. 
% Table \ref{tb:privacy-tradeoff} shows the results on 2dplanes dataset, and we defer the results for other datasets to Appendix \ref{appendix:experiment}. As we can see, DP-TKNN-Shapley shows a substantially better privacy-utility tradeoff compared to both DP-KNN-Shapley. In particular, DP-TKNN-Shapley maintains a high AUROC even when $\eps \approx 0.1$. The poor performance of DP-KNN-Shapley is due to its relatively high global sensitivity and not being able to incorporate subsampling techniques. 




% For instance, the AUROC for DP-KNN-Shapley drops quickly when $\eps<10^4$. In contrast, DP-TKNN-Shapley maintains a high AUROC even when $\eps \approx 0.1$. This improved tradeoff can be attributed to the fact that DP-TKNN-Shapley benefits from privacy amplification by subsampling, an advantage that DP-KNN-Shapley does not possess. However, even for the time-consuming version of DP-KNN-Shapley (with subsampling), DP-TKNN-Shapley still outperforms it; this superiority could be due to the relatively high global sensitivity of DP-KNN-Shapley.


% We assess the privacy-utility tradeoff of DP-TKNN-Shapley across a range of datasets. In particular, we plot the AUROC of mislabeled/noisy data detection tasks at various values of $\eps$, where $\eps$ is adjusted by modifying the magnitude of Gaussian noise in DP-TKNN-Shapley.

% As a baseline, we use an older version of KNN-Shapley, where it is possible to derive a non-trivial global sensitivity. We choose this version due to the difficulty in deriving a non-trivial global sensitivity of KNN-Shapley, as discussed in Section \ref{sec:difficulty-in-privatize-knn}. We denote this baseline as DP-KNN-Shapley (see Appendix \ref{appendix:background-more} for details).

% As shown in Figure \ref{fig:privacy-tradeoff}, DP-TKNN-Shapley demonstrates a significantly improved privacy-utility tradeoff compared to DP-KNN-Shapley. For example, the AUROC for DP-KNN-Shapley deteriorates rapidly when $\eps<10^4$. In contrast, DP-TKNN-Shapley maintains a robust AUROC even when $\eps \approx 0.1$. This enhancement in the tradeoff is attributable to the fact that DP-TKNN-Shapley leverages privacy amplification by subsampling, a benefit that DP-KNN-Shapley does not offer.

% We also included another baseline: a variant of DP-KNN-Shapley that employs the computationally intensive subsampling technique, as mentioned in Section \ref{sec:difficulty-in-privatize-knn}. The results show that DP-TKNN-Shapley still surpasses this computationally demanding version of DP-KNN-Shapley. This superiority could be due to the relatively high global sensitivity of DP-KNN-Shapley.



==> introduction.tex <==

\vspace{-1mm}
\section{Introduction}

\vspace{-1mm}
% \textbf{Data Valuation.} 
Data valuation is an emerging research area that seeks to measure the contribution of individual data sources to the training of machine learning (ML) models. Data valuation is essential in data marketplaces for ensuring equitable compensation for data owners, and in explainable ML for identifying influential training data. The importance of data valuation is underscored by the DASHBOARD Act introduced in the U.S. Senate in 2019 \citep{dashboardact}, which mandates companies to provide users with an assessment of their data's economic value. Moreover, OpenAI's Future Plan explicitly highlights ``the fair distribution of AI-generated benefits'' as a key question moving forward \citep{openaifuture}.


%Data valuation is an emerging research area that seeks to quantify the contribution of individual data to the training of machine learning (ML) models. This approach not only helps data owner understand how their data is being utilized, but is also essential for data collectors to make fair compensation or identify impactful training examples. In addition, recent DASHBOARD Act introduced in the U.S. Senate in 2019 mandates companies with over 100 million monthly active users to provide users with an assessment of their data's economic value. 

\vspace{-1mm}
\textbf{Data Shapley.} Inspired by cooperative game theory, \cite{ghorbani2019data,jia2019towards} initiated the study of using the Shapley value as a principled approach for data valuation. The Shapley value \citep{shapley1953value} is a famous solution concept from game theory for fairly assigning the total revenue to each player. 
In a typical scenario of data valuation, training data points are collected from different sources, and the data owner of each training data point can be regarded as ``player'' in a cooperative game. ``Data Shapley'' refers to the method of using the Shapley value as the contribution measure for each data owner. Since its introduction, many different variants of Data Shapley have been proposed \citep{jia2019efficient, ohrimenko2019collaborative, ghorbani2020distributional, wang2020principled, bian2021energy, kwon2022beta, lin2022measuring, wu2022davinz, karlavs2022data, wang2023data}, reflecting its effectiveness in quantifying data point contributions to ML model training. 


% In the context of data valuation for ML, training data points belongs to different data holders, and 

% ``player'' refers to the data holder of each training data point, and the methodology is dubbed as ``Data Shapley''. Since its introduction, many different variants of Data Shapley have been proposed \citep{jia2019efficient, ohrimenko2019collaborative, ghorbani2020distributional, wang2020principled, bian2021energy, kwon2022beta, lin2022measuring, wu2022davinz, karlavs2022data, wang2023data}, reflecting its effectiveness in quantifying data point contributions to ML model training. 

% The success of Data Shapley can be attributed in part to its unique axiomatic characterizations, which align with the natural fairness requirements of the ML context. 


% Inspired by cooperative game theory and economic principles,  the study of data valuation using the Shapley value, which
%  was initiated by \cite{ghorbani2019data} and \cite{jia2019towards}. This approach, dubbed ``Data Shapley'', evaluates the contribution of individual data point to the model output by calculating the Shapley value, which is the marginal difference in the model output (or a given utility function), averaged over all possible subsets of training sets. 
% Since then, several variant of Data Shapley have been proposed \citep{jia2019efficient, ohrimenko2019collaborative, ghorbani2020distributional, wang2020principled, bian2021energy, kwon2022beta, lin2022measuring, wu2022davinz, karlavs2022data, wang2023data}, reflecting its effectiveness in quantifying data point contributions to ML model training. The success of Data Shapley can be attributed in part to its unique axiomatic characterizations, which align with the natural fairness requirements of the ML context. 


\vspace{-1mm}
\textbf{KNN-Shapley.} 
While being a principled approach for data valuation, the exact calculation of the Shapley value is computationally prohibitive \citep{jia2019towards}. Various approximation algorithms for Data Shapley have been proposed \citep{jia2019towards, illes2019estimation, okhrati2021multilinear, burgess2021approximating, mitchell2022sampling, lin2022measuring, wang2023notegroup}, but these approaches still require substantial computational resources due to model retraining. Fortunately, a breakthrough by \cite{jia2019efficient} showed that computing the \emph{exact} Data Shapley for K-Nearest Neighbors (KNN), one of the oldest yet still popular ML algorithms, is surprisingly easy and efficient. 
KNN-Shapley quantifies data value based on KNN's Data Shapley score; it can be applied to large, high-dimensional CV/NLP datasets by calculating the value scores on the last-layer neural network embeddings. 
Owing to its superior efficiency and effectiveness in discerning data quality, KNN-Shapley is recognized as one of the most practical data valuation techniques nowadays \citep{pandl2021trustworthy}. It has been applied to various ML domains including active learning \citep{ghorbani2022data}, continual learning \cite{shim2021online}, NLP \citep{liang2020beyond, liang2021herald}, and semi-supervised learning \citep{courtnage2021shapley}. 

% , and has also demonstrated practical value in healthcare data valuation and ML pipeline data debugging.


% The release of data values to individuals can potentially compromise privacy if the training data includes sensitive information, as the value itself is a function of the individual data and the rest of the training data. Moreover, the privacy issue becomes more complex when considering a strong threat model where some data owners can collude (using their received data values) to identify a particular individual. However, the privacy concern of data valuation has received limited attention. We study this problem using Differential Privacy (DP), which is a quantifiable definition of privacy and provides provable guarantee against identifications of individuals.

\vspace{-1mm}
\textbf{Motivation: privacy risks in data valuation.} 
In this work, we study a critical, yet often overlooked concern in the deployment of data valuation: privacy leakage associated with data value scores released to data holders. The value of a single data point is always relative to other data points in the training set. This, however, can potentially reveal sensitive information about the rest of data holders in the dataset. This problem becomes even more complex when considering a strong threat model where multiple data holders collude, sharing their received data values to determine the membership of a particular individual. As data valuation techniques such as KNN-Shapley become increasingly popular and relevant in various applications, understanding and addressing the privacy implications of data valuation methods is of utmost importance. In this work, we study this critical issue through the lens of differential privacy (DP), a de-facto standard for privacy-preserving applications. 





%However, the data value itself is a function of the individual data and the rest training data. Can the release of data values to the individuals or data collectors compromise privacy if the training data includes sensitive information? This question has received little attention. We study this question using Differential Privacy (DP), which is a quantifiable definition of privacy and provides provable guarantee against identifications of individuals.

% However, the Shapley value is known to be computationally expensive. The number of utility function evaluations required by the exact SV calculation grows exponentially with the number of players, i.e., data points in the ML context. While there are many Monte Carlo-based Shapley value estimation algorithms have been proposed \citep{lundberg2017unified, jia2019towards, illes2019estimation, okhrati2021multilinear, burgess2021approximating, mitchell2022sampling, lin2022measuring, wang2023notegroup}, these approaches still require at least thousands of utility function evaluations. For ML tasks, evaluating the utility function itself (e.g., computing the validation accuracy of the ML model trained on a given dataset) is already computationally expensive, as it requires training a model from scratch. 

% \textbf{KNN-Shapley \& Its Applications.} 
% \textcolor{red}{However, the Shapley value is known to be computationally expensive.} Fortunately, \cite{jia2019efficient} found that computing the Data Shapley for K-Nearest Neighbors (KNN), one of the most classic yet still popular ML algorithms, is surprisingly easy and efficient. Specifically, \cite{jia2019efficient} show that for unweighted KNN classifiers, one can compute the \emph{exact} Shapley value for \emph{all of the $N$} data points in $O(N \log N)$ runtime in total, instead of the complex, $O(2^N)$ runtime calculation as suggested by the original formula. To the best of our knowledge, KNN is the \emph{only} commonly-used ML model for which the exact Data Shapley can be efficiently computed, referred to as `KNN-Shapley'. Owing to its superior computational efficiency and effectiveness in distinguishing data quality, KNN-Shapley has become one of the most popular and practical data valuation techniques. In the realm of ML research, for instance, \cite{ghorbani2022data} extends KNN-Shapley to active learning, \cite{shim2021online} employs it in a continual learning setting, \cite{liang2020beyond,liang2021herald} utilize KNN-Shapley for removing confusing samples in NLP applications, and \cite{courtnage2021shapley} adopts KNN-Shapley for data valuation in semi-supervised learning. Furthermore, KNN-Shapley has also proven to be highly practical in real-life applications: \cite{pandl2021trustworthy} demonstrates that KNN-Shapley is the \emph{only} practical data valuation technique for valuing large amounts of healthcare data, and \cite{karlavs2022data} builds the first data debugging system for end-to-end ML pipelines based on KNN-Shapley.

% Such a privacy concern does not exist in the traditional data marketplace \cite{} where all data are priced the same. However, a

% This issue has received relatively little attention in the research community and is often overlooked in practice. In this paper, we explore this question and provide both positive and negative answers, illustrating the potential privacy risks associated with the state-of-the-art data valuation technique, KNN-Shapley. 

\vspace{-1mm}
Our technical contributions are listed as follows.

\vspace{-1mm}
\underline{\textbf{Privacy Risks \& Challenges of Privatization for KNN-Shapley.}} We demonstrate that data value scores, specifically those computed by KNN-Shapley, indeed serve as a new channel for private information leakage, potentially exposing sensitive information about individuals in the dataset. We also highlight the technical challenges in converting the current KNN-Shapley technique into a differentially private version, emphasizing the need for a more privacy-friendly approach. 


%We also highlight a few challenges in privatizing the current KNN-Shapley technique, including the inconsistency between its recursive calculation and privacy analysis, which

% We propose a new data valuation method TKNN-Shapley and its private variant, which significantly improves the privacy-utility trade-off when releasing individual data values. Intuitively, training data that does not belong to the neighbors set of the query shall have a zero value. We realize this intuition by considering a threshold-based kNN(TKNN), which takes into account all neighbors within a pre-specified threshold of a test query, rather than the exact K nearest neighbors. We derive the closed form of Data Shapley for TKNN, which preserves the computational efficiency advantages of the original KNN-Shapley. Additionally, we demonstrate that by publishing a summary of statistics of the private dataset associated with each test example, we can  privately release all individual data values simultaneouly. 
 
\vspace{-1mm}
\underline{\textbf{TKNN-Shapley: an efficient, privacy-friendly data valuation technique.}} To address these privacy concerns, we propose a novel variant of KNN-Shapley called TKNN-Shapley. This new method considers an alternative form of KNN classifier called Threshold-KNN (TKNN) which takes into account all neighbors within a pre-specified threshold of a test example, rather than the exact K nearest neighbors. We derive the closed form of Data Shapley for TKNN (i.e., TKNN-Shapley), which achieves improved computational efficiency over the original KNN-Shapley. Crucially, TKNN-Shapley can be conveniently transformed into a differentially private version (DP-TKNN-Shapley). Such a DP variant satisfies favorable properties, including the capability to withstand collusion among data holders without compromising privacy guarantee. 

% Moreover, TKNN-Shapley can be easily converted into a differentially private version, which satisfies useful properties such as allowing collusion between data holders. 

% \tianhao{Table for the comparison between KNN/TKNN-Shapley}

\vspace{-1mm}
\underline{\textbf{Numerical experiments.}}
Our experiments highlight the robust performance of TKNN-Shapley across 13 datasets. Key observations include: (1) TKNN-Shapley surpasses KNN-Shapley in terms of computational efficiency; (2) DP-TKNN-Shapley significantly outperforms the naively privatized KNN-Shapley in terms of privacy-utility tradeoff; (3) even non-private TKNN-Shapley achieves comparable performance as the original KNN-Shapley in discerning data quality. 

% The differentially private version of TKNN-Shapley, termed as DP-TKNN-Shapley, significantly outperforms the naively privatized KNN-Shapley in terms of privacy-utility tradeoff.

\vspace{-1mm}
Overall, our work suggests that TKNN-Shapley, being a privacy-friendly, yet more efficient and effective alternative to the original KNN-Shapley, signifies a milestone toward practical data valuation.

% Overall, our work suggests that TKNN-Shapley is a privacy-friendly, yet more efficient and effective alternative to the original KNN-Shapley, signifies a milestone toward practical data valuation. 




% Overall, our work suggests that TKNN-Shapley is a promising alternative to the original KNN-Shapley given its computational advantage and privacy-friendly nature. 


% \subsection{Related Work and Novelty}
% Few literature considers the privacy risks of data valuation. \cite{tian2022private} consider the scenario where a trusted server does not exist and different users collaboratively compute each other's Shapley value without actually looking at the user's data points, with Multi-party Computation (MPC) technique. The privacy risks considered in \cite{tian2022private} are orthogonal to the one in this paper, and we can combine both techniques for end-to-end privacy protection. 
% Another line of works \cite{liu2021dealer, fallah2022optimal, cummings2022optimal, kang2023fair} considers the scenario where the data owners specify a privacy level and use the privacy level to adjust the data pricing mechanism correspondingly. 
% The unpublished manuscript by \cite{watson2022differentially} is the closest to our work. \cite{watson2022differentially} also studied the differentially private Shapley values of data points. However, instead of KNN-Shapley, they focus on privatizing the unrealistic, retrain-based Data Shapley. Moreover, their algorithm is highly restricted in the sense that the differential privacy guarantee requires the ``diminishing marginal'' assumption, which is not verifiable for most of the modern learning algorithms such as neural networks. 

==> motivation.tex <==

\begin{figure}[t]
    \setlength\intextsep{0pt}
    \setlength\abovecaptionskip{0pt}
    \setlength\belowcaptionskip{-10pt}
    \centering
    \includegraphics[width=0.85\textwidth]{image/flowchart_update.pdf}
    \caption{ 
    The potential privacy risks in data valuation arise from the dependency of the data value score $\phi_{z_i}$ on the rest of the dataset $D_{-z_i}$. Our goal is to privatize $\phi_{-z_i}(D_{-z_i})$ such that it provides strong differential privacy guarantee for the rest of the dataset $D_{-z_i}$. 
    % \tianhao{refine figure}
    }
    \label{Fig:threat-model}
\end{figure}

\vspace{-2mm}
% \section{Motivation: Data Value Scores Can Leak Privacy}
\section{Privacy Risks \& Challenges of Privatization for KNN-Shapley}
\label{sec:motivation}

\vspace{-1mm}
\textbf{Scenario.} 
Figure \ref{Fig:threat-model} illustrates the data valuation scenario and potential privacy leakages considered in our paper. Specifically, 
% in a typical scenario of data valuation, 
a centralized, trusted server collects data point $z_i$ from data owner $i$ for each $i \in [N]$. 
The central server's role is to provide each data owner $i$ with an assessment of their data's value, e.g., the KNN-Shapley value $\phi^{\knn}_{z_i}$. 
\textbf{A real life example:} Mayo Clinic has created a massive digital health patient data marketplace platform \citep{mayo}, where the patients submit part of their medical records onto the platform, and life science companies/labs pay a certain amount of money to purchase patients’ data. The platform's responsibility is to gauge the worth of the data of each patient (i.e., the data owner) to facilitate fair compensation. 

\vspace{-1mm}

\begin{wrapfigure}{R}{0.35 \textwidth}
    \setlength\intextsep{0pt}
    \setlength\abovecaptionskip{0pt}
    \setlength\belowcaptionskip{-10pt}
    \vspace{-5mm}
    \centering
    \includegraphics[width=0.35 \columnwidth]{image/privleak+miatable.pdf}
    \caption{ \textbf{Left:} Curves of KNN-Shapley of a fixed data point as a function of $K$ (the hyperparameter for KNN), with and without a particular nearby data point in the training set. 
    \add{\textbf{Right:} Results of AUROC of the MIA attack (detailed in Appendix \ref{appendix:mia}) on KNN-Shapley.}
    }
    \label{fig:leakpriv}
\end{wrapfigure}
The privacy risks associated with KNN-Shapley (as well as other data valuation techniques) arises from the fact that $\phi^{\knn}_{z_i}(D_{-z_i})$ depends on other data owners' data $D_{-z_i}$. Consequently, the data value score $\phi^{\knn}_{z_i}$ may inadvertently reveal private information (e.g., membership) about the rest of the dataset. The dependency of a data value score on the rest of the dataset is an unavoidable aspect of data valuation, as the value of a data point is inherently a relative quantity determined by its role within the complete dataset. 

% \tianhao{a few sentences about the practical scenario of the threat model}

\vspace{-1mm}
\begin{remark}[\textbf{Other privacy risks in data valuation}]
It is important to note that in this work, we do not consider the privacy risks of revealing individuals' data to the central server. This is a different type of privacy risk that needs to be addressed using secure multi-party computation (MPC) technique, and it should be used together with differential privacy in practice. In addition, to use KNN-Shapley or many other data valuation techniques, the central server needs to maintain a clean, representative validation set, the privacy of which is not considered by this paper. 
\end{remark}

\vspace{-1mm}
\textbf{Experiments for the source of privacy risks.} We illustrate the privacy risks of revealing data value scores with a concrete example, where we investigate the impact of removing a data point on the KNN-Shapley score of another data point that is close to the removed one. 
% Specifically, we first compute the KNN-Shapley score for a selected data point in the original dataset, and then repeat the process after removing one of its nearby data points. 
Specifically, we calculate the KNN-Shapley score for a chosen data point in the dataset, and then repeat the process after eliminating one of its nearby points from the dataset. 
% We show the results on CPU dataset \citep{cpudataset} in Figure \ref{fig:leakpriv}, and defer the results on additional datasets to Appendix \ref{appendix:experiment}. We can see from Figure \ref{fig:leakpriv} that there's a significant difference in KNN-Shapley score for the inspected data point depending on whether the nearby data point has been removed or not. 
The results in Figure \ref{fig:leakpriv} (on CPU dataset \citep{cpudataset}) show a substantial difference in the KNN-Shapley score of the investigated data point depending on whether the nearby data point has been removed. Additional results on other datasets can be found in Appendix \ref{appendix:knnsv-privrisk-score}.

\add{
\textbf{A Simple Membership Inference Attack (detailed in \ref{appendix:mia}).} 
Our observation demonstrates the potential for KNN-Shapley scores to leak membership information of other data points in the dataset. Analogous to the classic membership inference attack on ML model \cite{shokri2017membership}, in Appendix \ref{appendix:mia} we show an example of privacy attack where an adversary could infer the presence/absence of certain data points in the dataset based on the variations in the KNN-Shapley scores. The design is analogous to the membership inference attack against ML models via the \emph{likelihood ratio test} \citep{carlini2022membership}. 
Part of the AUROC score of the attack results are shown in Figure \ref{fig:leakpriv} (right). 
As we can see, our MIA attack can achieve a detection performance that is better than the random guess (0.5) for most of the settings. On some datasets, the attack performance can achieve $> 0.7$ AUROC. This demonstrates that privacy leakage in data value scores can indeed lead to non-trivial privacy attacks. 
This underscores the need for privacy safeguards in data valuation due to inherent privacy risks.} 

%\tianhao{make a stronger connection to MIA in appendix; refer to appendix}


% We consider the setting where there is a centralized, trusted server that collects data point $z_i$ from user $i$ for each $i \in [N]$. The centralized server maintains a validation set which we do not concern about its privacy in this paper. The centralized server will provide each user $i$ an assessment of the value of the user $i$'s data, which is the KNN-Shapley $\phi_{z_i}$ for user $i$'s data $z_i$. The privacy leakage from KNN-Shapley lies in the fact that $\phi_{z_i}(D)$ is a function of other users' data. This is intuitive since a data point's value is always relative to the full dataset it is in. \textbf{From now on, we change the notation to $\phi_{z_i}(D_{-z_i})$ to emphasize this dependency.} 

% \tianhao{Should stress that it is reasonable to assume that different users do NOT collude with each other. }

\vspace{-1mm}
\subsection{ Privatizing KNN-Shapley is Difficult }
\label{sec:difficulty-in-privatize-knn}

% As data valuation techniques, especially for KNN-Shapley, become increasingly popular and relevant in various applications, mitigating its privacy risks is of utmost importance. 

\vspace{-1mm}
The growing popularity of data valuation techniques, particularly KNN-Shapley, underscore the critical need to mitigate the inherent privacy risks. In the quest for privacy protection, Differential privacy (DP) \citep{dwork2006calibrating} has emerged as a leading framework. DP has gained considerable recognition for providing robust, quantifiable privacy guarantees, thereby becoming the de-facto choice in privacy protection. 
% However, while DP may seem like the ideal solution, its integration with KNN-Shapley is riddled with challenges. 
In this section, we introduce the background of DP and highlight the difficulties in constructing a differentially private variant for the current version of KNN-Shapley. 

% constructing a differentially private variant for a 
% adopting DP for data valuation is not a straightforward task.

% % Differential privacy (DP) is the \emph{most} widely accepted framework for reasoning about the privacy guarantees of an algorithm. It provides a robust and quantitative privacy guarantee and is the go-to solution for privacy protection. 
% In this section, we introduce the background of DP and highlight the difficulties in constructing a differentially private variant for the current version of KNN-Shapley. 

\vspace{-1mm}
\textbf{Background of Differential Privacy.} We use $D, D' \in \MS$ to denote two datasets with an unspecified size over space $\cX$. We call two datasets $D$ and $D'$ \emph{adjacent} (denoted as $D \sim D'$) if we can construct one by adding/removing one data point from the other.

% Differential privacy (DP) is a framework to reason about the privacy guarantees of randomized algorithms that make use of sensitive data \citep{dwork2006calibrating}. DP provides a robust and quantitative privacy guarantee and has been widely accepted as the \emph{only} framework for reasoning about the privacy guarantees of an algorithm. 
% Formally, 

\vspace{-0.5mm}
\begin{definition}[Differential Privacy \citep{dwork2006calibrating}] 
\label{def:DP}
For $\eps, \delta \ge 0$, a randomized algorithm $\M : \MS \rightarrow \cY$ is 
{\em $(\eps, \delta)$-differentially private} if for every pair of adjacent datasets $D \sim D'$ and for every subset of possible outputs $E \subseteq \cY$, we have
$
\Pr_{\M}[\M(D) \in E] \le e^\eps \Pr_{\M}[\M(D') \in E] + \delta 
$. 
% where the randomness is over the coin flips of $\M$. 
\end{definition}

\vspace{-1mm}
That is, $(\eps, \delta)$-DP requires that for all adjacent datasets $D, D'$, the output distribution $\M(D)$ and $\M(D')$ are close, where the closeness is measured by the parameters $\eps$ and $\delta$. 
In our scenario, we would like to modify data valuation function $\phi_{z_i}(D_{-z_i})$ to satisfy $(\eps, \delta)$-DP in order to protect the privacy of the rest of the dataset $D_{-z_i}$. 
Gaussian mechanism \citep{dwork2006our} is a common way for privatizing a function; it introduces Gaussian noise aligned with the function's \emph{global sensitivity}, which is the maximum output change when a single data point is added/removed from any given dataset.

% Gaussian mechanism is a common way of privatizing a function; it adds Gaussian noise proportional to the function's \emph{global sensitivity}, which measures the maximum possible change in the function's output when a single data point in an arbitrary dataset is added/removed. 

% A common way to achieve DP is Gaussian mechanism, which adds
% % by adding 
% Gaussian noise proportional to the function's \emph{global sensitivity}, which measures the maximum possible change in the function's output when a single data point in an arbitrary dataset is added/removed. 

\vspace{-1mm}

\begin{definition}[Gaussian Mechanism \citep{dwork2006our}]
\label{thm:gaussian}
Define the global sensitivity of a function $f: \MS \rightarrow \mathbb{R}^d$ as $\Delta_2(f) := \sup_{D \sim D'} \norm{ f(D) - f(D') }_2$. The Gaussian mechanism $\M$ with noise level $\sigma$ is then given by $\M(D) := f(D)+ \N \left(0, \sigma^2 \ind_d\right)$ where $\M$ is $(\eps, \delta)$-DP with $\sigma = \Delta_2(f) \sqrt{\log (1.25 / \delta)} / \eps$. 
\end{definition}


% \vspace{-1mm}
% \textbf{Challenges in making KNN-Shapley being differentially private (overview).} 

% However, the recursive nature of Theorem~\ref{thm:knn-shapley} 
% renders it incompatible with privacy analysis. We can summarize the reasons into two-fold. Firstly,  Theorem~\ref{thm:knn-shapley} 
% necessitates the privately release of $\phi^\knn_{z_{i+1}}(D_{-z_{i+1}})$ before releasing $\phi^\knn_{z_i}(D_{-z_i})$, resulting in a total of $N$ compositions of DP mechanisms. From composition, we know that the privacy loss grows at a rate of $O(\sqrt{N})$, leading to weak utility for a large
% dataset. Secondly, ``privacy amplification by subsampling'' \citep{balle2018privacy} is a powerful primitive extensively used  in privacy-preserving deep learning~\citep{abadi2016deep}. This technique first samples a subset from a private dataset and then apply the DP mechanism on the subset.


%  where the subsampling of a dataset amplifies the privacy guarantees due to the reduced probability of an individual's data being included.



% It is challenging to derive a (non-trivial) global sensitivity of $\phi^\knn_{z_i}(D_{-z_i})$. Moreover, in Appendix \ref{appendix:background-more} we show that the global sensitivity of $\phi^\knn_{z_i}(D_{-z_i})$ is at least $1/2 - 1/(2C)$ by constructing a specific pair of neighboring datasets. On the other hand, the magnitude of each $\phi^\knn_{z_i}$ is approximately $O(1/K)$. Hence, if we introduce random noise proportional to the global sensitivity, the resulting privatized data value score could substantially deviate from the non-private version, which makes the privatized data value scores have low utility. 
% \uline{\textbf{(2) Vulnerability to collusion:}} Even if a good global sensitivity bound for $\phi^\knn_{z_i}(D_{-z_i})$ can be derived, the privacy guarantee of releasing a noisy $\widehat \phi^\knn_{z_i}(D_{-z_i})$ to individual $i$ would heavily rely on the assumption that individuals do not share the noisy $\widehat \phi^\knn_{z_i}(D_{-z_i})$ with others. 
% % For example, if an adversary sees both $\widehat \phi^\knn_{z_1}(D_{-z_1})$ and $\widehat \phi^\knn_{z_2}(D_{-z_2})$, then the privacy guarantee for the rest of the dataset $D_{-\{z_1, z_2\}}$ is degraded. 
% % becomes fragile in the face of collusion where a group of individuals share their noisy $\phi^\knn_{z_i}(D_{-z_i})$, resulting in a breach of privacy guarantees. 
% \uline{\textbf{(3) Difficulty in incorporating privacy amplification by subsampling:}} ``Privacy amplification by subsampling'' \citep{balle2018privacy} is a technique where the subsampling of a dataset amplifies the privacy guarantees due to the reduced probability of an individual's data being included. Being able to incorporate such a technique is often important for achieving a decent privacy-utility tradeoff. However, the recursive nature of KNN-Shapley computation makes it hard to incorporate the subsampling techniques. 

















\vspace{-1mm}
\textbf{Challenges in making KNN-Shapley being differentially private (overview).} 
Here, we give an overview of the inherent difficulties in making the KNN-Shapley $\phi^{\knn}_{z_i}(D_{-z_i})$ (Theorem \ref{thm:knn-shapley}) to be differentially private, and we provide a more detailed discussion in Appendix \ref{appendix:background-more}. 
\uline{\textbf{(1) Large global sensitivity:}} 
% It is challenging to tightly bound the global sensitivity of $\phi^\knn_{z_i}(D_{-z_i})$. 
In Appendix \ref{appendix:background-more}, we show that the global sensitivity of $\phi^\knn_{z_i}(D_{-z_i})$ can significantly exceed the magnitude of $\phi^\knn_{z_i}$. Moreover, we prove that the global sensitivity bound cannot be further improved by constructing a specific pair of neighboring datasets that matches the bound. 
% is at least around $O(1)$ by constructing a specific pair of neighboring datasets. On the other hand, the magnitude of each $\phi^\knn_{z_i}$ is approximately $O(1/K)$. 
% Moreover, in Appendix \ref{appendix:background-more}, we show that the global sensitivity of $\phi^\knn_{z_i}(D_{-z_i})$ is at least around $O(1)$ by constructing a specific pair of neighboring datasets. On the other hand, the magnitude of each $\phi^\knn_{z_i}$ is approximately $O(1/K)$. 
Hence, if we introduce random noise proportional to the global sensitivity bound, the resulting privatized data value score could substantially deviate from its non-private counterpart, thereby compromising the utility of the privatized data value scores. 
%if we introduce random noise proportional to the global sensitivity, the resulting privatized data value score could substantially deviate from the non-private version, which makes the privatized data value scores have low utility. 
% \uline{\textbf{(2) Vulnerability to collusion:}} Even if a good global sensitivity bound for $\phi^\knn_{z_i}(D_{-z_i})$ can be derived, the privacy guarantee of releasing a noisy $\widehat \phi^\knn_{z_i}(D_{-z_i})$ to individual $i$ would heavily rely on the assumption that individuals do not share the noisy $\widehat \phi^\knn_{z_i}(D_{-z_i})$ with others. 
% % For example, if an adversary sees both $\widehat \phi^\knn_{z_1}(D_{-z_1})$ and $\widehat \phi^\knn_{z_2}(D_{-z_2})$, then the privacy guarantee for the rest of the dataset $D_{-\{z_1, z_2\}}$ is degraded. 
% % becomes fragile in the face of collusion where a group of individuals share their noisy $\phi^\knn_{z_i}(D_{-z_i})$, resulting in a breach of privacy guarantees. 
\uline{\textbf{(2) Difficulty in incorporating privacy amplification by subsampling:}} ``Privacy amplification by subsampling'' \citep{balle2018privacy} is a technique where the subsampling of a dataset amplifies the privacy guarantees due to the reduced probability of an individual's data being included. Being able to incorporate such a technique is often important for achieving a decent privacy-utility tradeoff. 
However, the recursive nature of KNN-Shapley computation makes it hard to incorporate the subsampling techniques. 
% In Appendix \ref{appendix:background-more}, we show that the release of \emph{all} $(\phi^\knn_{z_i})_{z_i \in D}$ requires a runtime of $\widetilde{O}(N^2)$ if we incorporate the subsampling technique, which is a significant increase in computational demand compared to the non-private KNN-Shapley. 

% Recall that in a practical scenario of data valuation, the central server typically wants to release $\phi^\knn_{z_i}$ for \emph{all} $z_i \in D$. 

% However, to apply the subsampling technique, we first need to create a subsampled dataset and compute the KNN-Shapley for the target data point $z_i$. This operation requires a runtime of $\widetilde{O}(N)$ for the release of \emph{each} $\phi^\knn_{z_i}$, resulting in a final runtime of $\widetilde{O}(N^2)$ for the release of \emph{all} $(\phi^\knn_{z_i})_{z_i \in D}$. This is a significant increase in computational demand compared to the non-private KNN-Shapley. The recursive nature of KNN-Shapley computation further complicates the attempt of improving the computational efficiency. 

\vspace{-1mm}
These challenges underscore the pressing need for new data valuation techniques that retain the efficacy and computational efficiency of KNN-Shapley, while being amenable to privatization. 



% These challenges underscore the need for new data valuation approaches that maintain the effectiveness and computational efficiency of KNN-Shapley, while being easily augmented to be differentially private. 

% \tianhao{For Yuqing: you can mention two points: (1) Deriving the global sensitivity for $\phi^\knn_{z_i}(D_{-z_i})$ is hard; (2) we want to release $\phi^\knn_{z_i}(D_{-z_i})$ for all $i$, but since the computation of $\phi^\knn_{z_i}(D_{-z_i})$ is a recursive formula, we cannot benefit from privacy amplification via subsampling techniques without sacrificing computational efficiency.}


==> preliminary.tex <==

\vspace{-3mm}
%\section{Preliminary}
%\section{Data Valuation: A Function of the Rest of the Training Set}

\section{Background of Data Valuation}

\vspace{-3mm}
In this section, we formalize the data valuation problem for ML, and review the method of Data Shapley and KNN-Shapley. 

\vspace{-1mm}
% \subsection{Data Valuation for Machine Learning}
\textbf{Setup \& Goal.} Suppose we have a dataset $D := \{ z_i \}_{i=1}^N$ containing $N$ labeled data points where each data point $z_i := (x_i, y_i)$ is collected from a data owner $i$. The objective of data valuation is to assign a score to each training data point $z_i$ in a way that reflects its value or quality for ML model training. 
More formally, we want to find a score vector $(\phi_{z_i})_{i=1}^N$ where each $\phi_{z_i}$ represents the value of the data point $z_i$. The value of a data point is always relative to the rest of the data points in the dataset. Hence, $\phi_{z_i}$ is always a function of $D_{-z_i}$ where we denote the leave-one-out dataset $D_{-z} := D \setminus \{z\}$. We write $\phi_{z_i}(D_{-z_i})$ when we want to stress the dependency of a data value score with the rest of the data points. 

\vspace{-1mm}
\textbf{Utility Function.} 
Most of the existing data valuation techniques are centered on the concept of \emph{utility function}, which maps an input dataset to a score indicating the usefulness of the training set. A common choice for utility function is the validation accuracy of a model trained on the input training set. Formally, for a training set $S$, a utility function $\U(S) := \metric(\A( S ))$, where $\A$ is a learning algorithm that takes a dataset $S$ as input and returns a model; $\metric(\cdot)$ is a metric function that evaluates the performance of a given model, e.g., the classification accuracy on a hold-out validation set. 

% The goal of data valuation is to partition $\U(D)$, the utility of the entire dataset, to the individual data point $z \in D$. 


\vspace{-2mm}
\subsection{The Shapley Value}

\vspace{-1mm}
The Shapley value (SV) \citep{shapley1953value} is a classic concept from game theory to attribute the total gains generated by the coalition of all players. At a high level, it appraises each point based on the (weighted) average utility change caused by adding the point into different subsets of the training set. Formally, given a utility function $\U(\cdot)$ and a training set $D$, the Shapley value of a data point $z \in D$ is defined as 
\begin{small}
\begin{align}
&\phi_z\left( D_{-z}; \U \right) := \frac{1}{N} \sum_{k=1}^{N} {N-1 \choose k-1}^{-1} \sum_{S \subseteq D_{-z}, |S|=k-1} \left[ \U(S \cup \{z\}) - \U(S) \right]
\label{eq:shapley-formula}
\end{align}
\end{small}

\vspace{-1mm}
For notation simplicity, when the context is clear, we omit the utility function and/or leave-one-out dataset, 
and simply write $\phi_z(D_{-z})$, $\phi_z(\U)$ or $\phi_z$ depending on the dependency we want to stress. 
The popularity of the Shapley value is attributable to the fact that it is the \emph{unique} data value notion satisfying four axioms: Dummy player, Symmetry, Linearity, and Efficiency. We refer the readers to \citep{ghorbani2019data, jia2019towards} and the references therein for a detailed discussion about the interpretation and necessity of the four axioms in the ML context. Here, we introduce the \emph{linearity} axiom which will be used later. 

\begin{theorem}[Linearity of the Shapley value \cite{shapley1953value}]
\label{thm:linearity}
For any of two utility functions $\U_1, \U_2$ and any $\alpha_1, \alpha_2 \in \R$, we have $\phi_{z} \left( \alpha_{1} \U_{1}+\alpha_{2} \U_{2}\right)=\alpha_{1} \phi_z\left(\U_{1}\right)+$ $\alpha_{2} \phi_z\left( \U_{2}\right)$.
\end{theorem}

\vspace{-1mm}
\subsection{KNN-Shapley}

\vspace{-1mm}
Formula (\ref{eq:shapley-formula}) suggests that the exact Shapley value can be computationally prohibitive in general, as it requires evaluating $\U(S)$ for all possible subset $S \subseteq D$. Surprisingly, \citep{jia2019efficient, wang2023noteknn} showed that for KNN, the computation of the exact Data Shapley score is highly efficient. 
Following its introduction, KNN-Shapley has rapidly gained attention and follow-up works across diverse areas of machine learning \cite{ghorbani2022data, liang2020beyond, liang2021herald, courtnage2021shapley}. In particular, it has been recognized by recent studies as ``the most practical data valuation technique capable of handling large-scale data effectively'' \citep{pandl2021trustworthy, karlavs2022data}. 








% Specifically, consider a set of training data points $D = \{ z_i = (x_i, y_i)\}_{i=1}^{N}$ and a validation set $\Dval = \{ (x_{i}^{(\test)}, y_{i}^{(\test)}) \}_{i=1}^{N_\test}$. 
% Let $S \subseteq D$ be a subset of training data. We denote $\pi^{(S)}(i; x^{(\test)})$ the index (within $D$) of the $i$th closest data point in $S$ to $x^{(\test)}$. 
% The distance is measured through some appropriate metric, which we use $\ell_2$ distance throughout this paper without loss of generality. 
% Thus, $(x_{\pi^{(S)}(1; x^{(\test)})}, x_{\pi^{(S)}(2; x^{(\test)})}, \ldots, x_{\pi^{(S)}( |S| ; x^{(\test)})})$ is a reordering of the training instances in $S$ with respect to their distance from $x^{(\test)}$. When the context is clear, we omit the argument $x^{(\test)}$ and simply write $\pi^{(S)}(i)$. 
% As we mentioned earlier, the utility function $\U(\cdot)$ is usually defined as the validation accuracy of a model trained on the input training set. 







\vspace{-1mm}
Specifically, the performance of an unweighted KNN classifier is typically evaluated by its validation accuracy. For a given validation set $\Dval = \{ z_i^{(\test)}\}_{i=1}^{N_\test}$, 
% . The performance of an unweighted KNN classifier is typically evaluated by its validation accuracy on $\Dval$. Hence, for a non-empty training set $S$, 
we can define KNN's utility function $\U^\knn_{\Dval}$ on a non-empty training set $S$ as $\U^\knn_{\Dval}(S) := \sum_{\zval \in \Dval} \U^\knn_{\zval}(S)$, where
\begin{small}
\begin{align}
\U^\knn_{\zval}(S) &:= \frac{1}{\min(K, |S|)} \sum_{j=1}^{\min(K, |S|)} \ind[y_{ \pi^{(S)}(j; \xval) } = y^{(\test)}]
\label{eq:new-util-func}
\end{align}
\end{small}
is the likelihood of a (soft-label) KNN-classifier in predicting the correct label for a validation point $\zval = (x^{(\test)}, y^{(\test)}) \in \Dval$. In (\ref{eq:new-util-func}), $\pi^{(S)}(i; x^{(\test)})$ is the index of the $i$th closest data point in $S$ to $x^{(\test)}$. When $|S|=0$, $\U^\knn_{\zval}(S)$ is set to the accuracy by random guessing. The distance is measured through suitable metrics such as $\ell_2$ distance. 
Here's the main result in \cite{jia2019efficient, wang2023noteknn}:

% \begin{align}
% \U^\knn_{\zval}(S) &:= 
% \begin{cases} 
%       1/C & |S|=0 \\
%       \frac{1}{\min(K, |S|)} \sum_{j=1}^{\min(K, |S|)} \ind[y_{ \pi^{(S)}(j) } = y^{(\test)}] & |S|>0 
% \end{cases}
% \label{eq:new-util-func}
% \end{align}

% the utility $1/C$ is the accuracy by random guessing, where $C$ is the number of classes for the corresponding classification task. The distance is measured through metrics such as $\ell_2$ distance. 




% the utility function $\U^\knn_{\Dval}$ of an unweighted, soft-label KNN classifier trained on a data subset $S \subseteq D$ is its aggregated prediction accuracy on each validation data point $\zval \in \Dval$, i.e.,
% $\U^\knn_{\Dval}(S) := \sum_{\zval \in \Dval} \U^\knn_{\zval}(S)$ where 
% \begin{align}
% \U^\knn_{\zval}(S) &:= 
% \begin{cases} 
%       1/C & |S|=0 \\
%       \frac{1}{\min(K, |S|)} \sum_{j=1}^{\min(K, |S|)} \ind[y_{ \pi^{(S)}(j) } = y^{(\test)}] & |S|>0 
% \end{cases}
% \label{eq:new-util-func}
% \end{align}
% is the likelihood of a soft-label KNN-classifier in predicting the correct label $y^{(\test)}$ for $x^{(\test)}$. 
% In (\ref{eq:new-util-func}), $\pi^{(S)}(i; x^{(\test)})$ is the index (within $D$) of the $i$th closest data point in $S$ to $x^{(\test)}$. When $|S|=0$, the utility $1/C$ is the accuracy by random guessing, where $C$ is the number of classes for the corresponding classification task. The distance is measured through metrics such as $\ell_2$ distance. 



% throughout this paper without loss of generality.

% % defined as its prediction accuracy, i.e., 
% % \begin{align}
% % \U_{\Dval}(S) &:= \sum_{(x^{(\test)}, y^{(\test)}) \in \Dval} \U_{\zval}(S) \label{eq:old-util-all} \\
% % \text{where~~}
% % \U_{\zval}(S) &:= 
% % \begin{cases} 
% %       1/C & |S|=0 \\
% %       \frac{1}{\min(K, |S|)} \sum_{j=1}^{\min(K, |S|)} \ind[y_{ \pi^{(S)}(j) } = y^{(\test)}] & |S|>0 
% % \end{cases}
% % \label{eq:new-util-func}
% % \end{align}
% where $\pi^{(S)}(i; x^{(\test)})$ is the index (within $D$) of the $i$th closest data point in $S$ to $x^{(\test)}$. When $|S|=0$, we set the utility as the accuracy of random guess $1/C$, where $C$ is the number of classes for the corresponding classification task. The distance is measured through some appropriate metric, which we use $\ell_2$ distance throughout this paper without loss of generality.

% This utility function corresponds to the prediction accuracy of an unweighted, soft-label KNN classifier. When $|S|=0$, we set the utility as the accuracy of random guess. 




% \begin{algorithm}[htbp]
% \caption{KNN-Shapley}
% \label{alg:kNN}
% \begin{algorithmic}[1]
% \STATE{\textbf{Input}: Dataset $D:=\{z_i\}_{i=1}^N$, validation set $D^{(\text{val})}$}
% \FOR{$\zval \in \U_{\Dval}$}
% \STATE{$S:=$ Top $K$ nearest neighbors of $\zval$}
% \STATE{$\U^\knn_{\zval}(S)=\frac{1}{\min(K, |S|)} \sum_{j=1}^{\min(K, |S|)} \ind[y_{ \pi^{(S)}(j) } = y^{(\test)}] $}
% \ENDFOR
% \STATE{\textbf{Return} }
% \end{algorithmic}
% \vspace{-1mm}
% \end{algorithm}

\begin{theorem}[KNN-Shapley \citep{jia2019towards, wang2023noteknn} (simplified version)]
\label{thm:knn-shapley}
Consider the utility function in (\ref{eq:new-util-func}). 
Given a validation data point $\zval = (x^{(\test)}, y^{(\test)})$ and a distance metric $d(\cdot, \cdot)$, if we sort the training set $D = \{z_i = (x_i, y_i)\}_{i=1}^N$ according to $d(x_i, x^{(\test)})$ in ascending order, then the Shapley value of each data point $\phi^\knn_{z_i}$ corresponding to utility function $\U^\knn_{\zval}$ can be computed recursively as follows:
\begin{align*}
\phi^\knn_{z_N} := f_N(D), ~~\mathrm{and}~~
\phi^\knn_{z_i} := \phi^\knn_{z_{i+1}} + f_i(D)~~~\text{for }i=1, \ldots, N-1
\end{align*}
where the exact form of functions $f_i(D)$ can be found in Appendix \ref{appendix:background-more}. 

\vspace{-1mm}
\emph{\textbf{Runtime:}} the computation of all Shapley values $(\phi^\knn_{z_1}, \ldots, \phi^\knn_{z_N})$ can be achieved in $O(N \log N)$ runtime in total (dominated by the sorting data points in $D$). 

\vspace{-1mm}
\emph{\textbf{The Shapley value corresponding to full validation set:}} for a validation set $\Dval$, recall that $\U^\knn_{\Dval}(S) := \sum_{\zval \in \Dval} \U^\knn_{\zval}(S)$. 
One can compute the Shapley value corresponding to $\U^\knn_{\Dval}$ by summing each $\phi^\knn_{z_i} \left(\U^\knn_{\zval} \right)$, i.e., 
$
\phi^\knn_{z_i} \left(\U^\knn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\knn_{z_i} \left(\U^\knn_{\zval} \right)
$. 
\end{theorem}
% \begin{theorem}[KNN-Shapley (simplified) \citep{wang2023noteknn}]
% \label{thm:knn-shapley}
% Consider the utility function in (\ref{eq:new-util-func}). Given the test data point $(x^{(\test)}, y^{(\test)})$, assume that the input dataset $D = \{z_i = (x_i, y_i)\}_{i=1}^N$ is sorted according to $\norm{x_i - x^{(\test)}}$ in ascending order. Then, the Shapley value of each training point $\phi^\knn_{z_i}(D_{-z_i})$ can be calculated recursively as follows: 
% \begin{small}
% \begin{align*}
%     \phi^\knn_{z_N}  &= \frac{\ind[N \ge 2]}{N} \left( \ind[y_N = y^{(\test)}] - \frac{ \sum_{i=1}^{N-1} \ind[y_i = y^{(\test)}] }{N-1} \right) \left( \sum_{j=1}^{ \min(K, N) - 1 } \frac{1}{j+1} \right) + \frac{1}{N} \left( \ind[y_N = y^{(\test)}] - \frac{1}{C} \right) \\
%     \phi^\knn_{z_i}  &= \phi^\knn_{z_{i+1}} + 
%     \frac{ \ind[y_i = y^{(\test)}] - \ind[y_{i+1} = y^{(\test)}] }{N-1} 
%     \left[
%     \sum_{j=1}^{\min(K, N)} \frac{1}{j} 
%     + \frac{\ind[N \ge K]}{K} \left( \frac{ \min(i, K) \cdot (N-1) }{i} - K
%     \right)
%     \right]
% \end{align*}
% \end{small}
% \end{theorem}

\vspace{-1mm}
Theorem \ref{thm:knn-shapley} tells that for any validation data point $\zval$, we can compute the \emph{exact} Shapley value $\phi^\knn_{z_i} \left(D_{-z_i}; \U^\knn_{\zval} \right)$ for \emph{all} $z_i \in D$ by using a recursive formula within a total runtime of $O(N \log N)$. After computing the Shapley value $\phi^\knn_{z_i} \left(\U^\knn_{\zval} \right)$ for each $\zval \in \Dval$, one can compute the Shapley value corresponding to the full validation set by simply taking the sum of each $\phi^\knn_{z_i} \left(\U^\knn_{\zval} \right)$, due to the linearity property (Theorem \ref{thm:linearity}) of the Shapley value. 

% We can easily see that after sorting the training data points according to their distances to $\zval$, \emph{all of} $(\phi^\knn_{z_1}, \ldots, \phi^\knn_{z_N})$ can be computed within $O(N)$ time, hence the overall time complexity is $O(N \log N)$ (i.e., the runtime is dominated by the step of sorting the training set). 
\begin{remark}[\textbf{Criteria of Computational Efficiency}]
As prior data valuation literature \citep{ghorbani2019data}, we focus on the total runtime required to release \emph{all} data value scores $(\phi^\knn_{z_1}, \ldots, \phi^\knn_{z_N})$. This is because in a practical data valuation scenario (e.g., profit allocation), we rarely want to compute the data value score for only a single data point; instead, a typical objective is to compute the data value scores for all data points within the training set. 
\label{remark:runtime}
\end{remark}

% \textbf{Releasing the Shapley value when using the full validation set.} 
% After computing the Data Shapley score $\phi^\knn_{z_i} \left(\U^\knn_{\zval} \right)$ for each $\zval \in \Dval$, one can compute the Data Shapley corresponding to the utility function $\U_{\Dval}$ on the overall validation set $\Dval$ through the linearity property (Theorem \ref{thm:linearity}) of the Shapley value, i.e., 
% $
% \phi^\knn_{z_i} \left(\U^\knn_{\Dval} \right) = \sum_{\zval \in \Dval} \phi^\knn_{z_i} \left(\U^\knn_{\zval} \right)
% $. 


==> table_privacyfull.tex <==

\begin{table*}[t]
\setlength\intextsep{0pt}
\setlength\abovecaptionskip{2pt}
% \setlength\belowcaptionskip{-10pt}
\centering
\resizebox{\textwidth}{!}{ 
\begin{tabular}{cccccccc} \toprule
\textbf{}                          & \textbf{}       & \multicolumn{3}{c}{\textbf{Mislabeled Data Detection}}                                                                                                                                                            & \multicolumn{3}{c}{\textbf{Noisy Data Detection}}                                                                                                                                                                 \\ \midrule
\textbf{Dataset}                   & \textbf{$\eps$} & \textbf{\begin{tabular}[c]{@{}c@{}}DP-TKNN-Shapley\\ (ours)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DP-KNN-Shapley\\ (no subsampling)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DP-KNN-Shapley\\ (with subsampling)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DP-TKNN-Shapley\\ (ours)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DP-KNN-Shapley\\ (no subsampling)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DP-KNN-Shapley\\ (with subsampling)\end{tabular}} \\ \midrule
\multirow{3}{*}{\textbf{2dplanes}} & \textbf{0.1} & 0.852 (0.009)                   & 0.494 (0.016)              & 0.703 (0.007)                 & 0.678 (0.025)         & 0.525 (0.013)                & 0.591 (0.008)                 \\
                                   & \textbf{0.5} & 0.887 (0.005)                   & 0.504 (0.002)              & 0.749 (0.003)                 & 0.726 (0.021)         & 0.511 (0.032)                & 0.66 (0.004)                  \\
                                   & \textbf{1}   & 0.894 (0.004)                   & 0.502 (0.011)              & 0.763 (0.002)                 & 0.776 (0.015)         & 0.518 (0.039)                & 0.668 (0.003)                 \\ \midrule
\multirow{3}{*}{\textbf{phoneme}}  & \textbf{0.1} & 0.817 (0.012)                   & 0.515 (0.018)              & 0.714 (0.006)                 & 0.645 (0.065)         & 0.512 (0.054)              & 0.562 (0.007)                 \\
                                   & \textbf{0.5} & 0.839 (0.003)                   & 0.521 (0.02)               & 0.741 (0.004)                 & 0.711 (0.011)         & 0.502 (0.012)              & 0.619 (0.002)                 \\
                                   & \textbf{1}   & 0.839 (0.002)                   & 0.503 (0.02)               & 0.766 (0.004)                 & 0.714 (0.009)         & 0.512 (0.034)              & 0.626 (0.002)                 \\ \midrule
\multirow{3}{*}{\textbf{CPU}}      & \textbf{0.1} & 0.877 (0.06)                    & 0.493 (0.013)              & 0.835 (0.003)                 & 0.742 (0.169)         & 0.501 (0.061)              & 0.564 (0.008)                 \\
                                   & \textbf{0.5} & 0.944 (0.009)                   & 0.499 (0.01)               & 0.93 (0.001)                  & 0.771 (0.026)         & 0.516 (0.011)              & 0.621 (0.007)                 \\
                                   & \textbf{1}   & 0.95 (0.003)                    & 0.503 (0.017)              & 0.935 (0.001)                 & 0.783 (0.025)         & 0.591 (0.088)              & 0.628 (0.006)                 \\ \bottomrule 
\end{tabular}
}
\caption{ 
Privacy-utility tradeoff of DP-TKNN-Shapley and DP-KNN-Shapley for mislabeled/noisy data detection task on 3 datasets of full size we use in the main paper. The full size of 2DPlanes, Phoneme, and CPU dataset is around 40,000, 5,000, and 8,000. 
We set $\delta = 10^{-5}$ and we show the AUROC at different privacy budgets $\eps$; the higher the AUROC is, the better the method is. We show the standard deviation of AUROC across 5 independent runs in (). 
}
\end{table*}



